A Unified Analysis of Variational Inequality Methods: Variance Reduction, Sampling, Quantization and Coordinate Descent

In this paper, we present a unified analysis of methods for such a wide class of problems as variational inequalities, which includes minimization problems and saddle point problems. We develop our analysis on the modified Extra-Gradient method (the classic algorithm for variational inequalities) and consider the strongly monotone and monotone cases, which corresponds to strongly-convex-strongly-concave and convex-concave saddle point problems. The theoretical analysis is based on parametric assumptions about Extra-Gradient iterations. Therefore, it can serve as a strong basis for combining the already existing type methods and also for creating new algorithms. In particular, to show this we develop new robust methods, which include methods with quantization, coordinate methods, distributed randomized local methods, and others. Most of these approaches have never been considered in the generality of variational inequalities and have previously been used only for minimization problems. The robustness of the new methods is also confirmed by numerical experiments with GANs.

==> include/RGEM.tex <==
\section{Метод экстраполяции случайного градиента}
\label{RGEM}
В данном параграфе рассмотрим \ev{метод экстраполяции случайного градиента}~\cite{lan2018random}. 
% Для ускорения в предложенном методе используется сэмплированный метод отрицательных моментов, котрый комбинирует в себе метод отрицательных моментов и новую схему двойного сэмплинга. Мы рассматриваем данный метод так как для него доказана наилучшая известная оценка скорости сходимости в терминах обращений к оракулу для сильновыпуклых задач \cite{zhou2018direct}. 
Отметим, что данный метод не требует пересчёта градиента на каждой итерации, необходимо пересчитывать только одну его компоненту на каждой итерации, что \ev{значительно} сокращает вычисления, особенно для задач большой размерности. Так как данный метод не является прямо-двойственным, то \ev{необходимо применять} алгоритм~\ref{alg_saga} к регуляризованной задаче.

% АГ: А ГДЕ В ЭТОМ АЛГОРИТМЕ ПРОЕКТИРОВАНИЕ? ВЕДЬ У НАС НЕОТРИЦАТЕЛЬНЫЕ МНОЖИТЕЛИ... ПО ИДЕЕ ГДЕ-ТО СРЕЗКИ НАДО СТАВИТЬ...

% ЕСЛИ ЧЕСТНО, ТО Я НЕ ПОНЯЛ, ПОЧЕМУ В ИТОГЕ ОСТАЛСЯ МЕТОД SAGA :( ВРОДЕ ХОТЕЛИ ЕГО ЗАМЕНИТЬ МЕТОДОМ RGEM ИЗ СТАТЬИ LAN-ZHOU \url{http://pwp.gatech.edu/guanghui-lan/wp-content/uploads/sites/330/2017/11/PAGED20171112ext.pdf}... ЗАМЕНИТЬ ХОТЕЛИ РОВНО ПОТОМУ, ЧТО В   SAGA НЕ ПРОРАБОТАНА НЕОТРИЦАТЕЛЬНОСТЬ ПЕРЕМЕННЫХ...
%\pd{underline и overline плоховато видно. предлагаю земенить на underline и overline}
    \begin{algorithm}
		\caption{Метод экстраполяции случайного градиента (RGEM)}\label{alg_saga}
		\begin{algorithmic}[1]
			\Require Параметры $\alpha$, $\eta$, $\tau$, $\{\theta_t\}_{t=1}^{N}$
			
			\State $\boldsymbol{\lambda}^0 := \mathbf{0}$
			\State $\underline{\boldsymbol{\lambda}}_i^0 := \boldsymbol{\lambda}^0$, $i = 1, \, \ldots, \, n$
			\State $y_{-1} = y_0 = \mathbf{0}$
			\For{$t=1, \, \ldots, \, N$}
    			\State 
    			\ev{Выбрать случайным образом}
    			%Случайно сгенерировать 
    			$k_t$ из множества $\{1, \, \ldots, \, n\}$ равномерно по всем значениям
    			\State $\tilde{\mathbf{y}}^t_k := \mathbf{y}^{t-1}_k + \alpha (\mathbf{y}^{t-1}_k - \mathbf{y}^{t-2}_k), \quad k = 1, \, \ldots, \, n$
    			\State $\boldsymbol{\lambda}^t := \left[\eta \boldsymbol{\lambda}^{t-1} - \frac{1}{n} \sum\limits_{k = 1}^n \tilde{\mathbf{y}}_k^t \right]_{+} / (\delta + \eta)$\\
    			
    			\State $\underline{\boldsymbol{\lambda}}_{k_t}^t := \left (\boldsymbol{\lambda}^t + \tau \underline{\boldsymbol{\lambda}}_{k_t}^{t-1} \right ) / (1 + \tau)$
    			\State $\underline{\boldsymbol{\lambda}}_{k}^t := \underline{\boldsymbol{\lambda}}_{k}^{t-1}$, $k \in \{1, \, \ldots \, n\} \setminus \{k_t\}$\\
    			\State $\mathbf{y}^t_{k_t} := \mathbf{b} - n \mathbf{C}_{k_t} x_{k_t}(\underline{\boldsymbol{\lambda}}_{k_t}^t)$
    			\State $\mathbf{y}^t_{k} := \mathbf{y}^{t-1}_{k}$, $k \in \{1, \, \ldots, \, n\} \setminus \{k_t\}$
    			
            \EndFor
            \State $\overline{\boldsymbol{\lambda}}^N := \left(\sum\limits_{t = 0}^{N-1} \theta_t \boldsymbol{\lambda}^t\right) / \sum\limits_{t = 1}^{N} \theta_t$
			\State\Return $\overline{\boldsymbol{\lambda}}^N$
		\end{algorithmic}
	\end{algorithm}
Параметры $\alpha$, $\eta$, $\tau$ и $\theta_t$ выбираются следующим образом:
\begin{equation} \label{params1}
\overline{\alpha} = 1 - \frac{1}{n + \sqrt{n^2 + 16 n L / \delta}},
\end{equation}
\begin{equation} \label{params}
\alpha = n \overline{\alpha}, \quad \eta = \frac{\delta \overline{\alpha}}{1 - \overline{\alpha}}, \quad \tau = \frac{1}{n (1 - \overline{\alpha})} - 1, \quad
\theta_t = \overline{\alpha}^{-t}.
\end{equation}
%Определим проксимальную функцию
%\begin{equation} \label{prox}
%P(\boldsymbol{\lambda}^1, \boldsymbol{\lambda}^2) = %\frac{1}{2} \|\boldsymbol{\lambda}^2\|_2^2 - %\left[\frac{1}{2} \|\boldsymbol{\lambda}^1\|_2^2 + %\langle\boldsymbol{\lambda}^1, %\boldsymbol{\lambda}^2 - %\boldsymbol{\lambda}^1\rangle\right]
%\end{equation}


\subsection{Распределённый метод}
В данной секции опишем распределённую версию рассмотренного метода. Для начала отметим, что векторы~$\underline{\boldsymbol{\lambda}}_1^0, \, \ldots, \, \underline{\boldsymbol{\lambda}}_n^0$ хранятся у соответствующих пользователей и влияют на формирование оптимального значения трафика для соответствующего пользователя. Как было отмечено при описании распределённого БГМ, на определение оптимального трафика пользователя влияют только цены соединений, \ev{через} которые данный пользователь \ev{обменивается пакетами}. Поэтому можно считать, что в векторе~$\underline{\boldsymbol{\lambda}}_k^t$ ненулевые только те компоненты, номера которых совпадают с номерами используемых соединений. 

Опишем распредел\ev{ё}нный алгоритм на $t$ итерации:

1. \ev{Используя} информацию, собранную с пользователей \ev{на} предыдущей итерации соединение~$j$ \ev{вычисляет} 
$$
\tilde{y}^t_{k,j} := y^{t-1}_{k,j} + \alpha 
\left ( y^{t-1}_{k,j} - y^{t-2}_{k,j} \right ) = b_{j}-nC_{k}^j x_{k} \left (\underline{\boldsymbol{\lambda}}_k^{t-1} \right ) + \alpha 
\left ( nC_{k}^j x_{k}(\underline{\boldsymbol{\lambda}}_k^{t-2}) - nC_{k}^j x_{k} \left (\underline{\boldsymbol{\lambda}}_k^{t-1} \right ) \right ).
$$
\ev{З}аметим, что в силу определения матрицы $C$ соединению $j$ нужна информация только 
\ev{от} пользователей, которые \ev{обмениваются пакетами через это соединение.}%его используют. 

2. Далее соединение $j$ меняет цену по следующему правилу\ev{:} 
$$
\lambda_j^t = \left[\eta \lambda_j^{t-1} - \frac{1}{n} \sum_{k=1}^n \tilde{y}_{k, \, j}^t \right]_{+} / (\delta + \eta).
$$
    	
3. \ev{О}дин из пользователей $k_t$ реагирует на изменение цен и в качестве локального вектора цен сохраняет 
 $$\underline{\boldsymbol{\lambda}}_{k_t}^t = 
 \left (\boldsymbol{\lambda}^t + \tau \underline{\boldsymbol{\lambda}}_{k_t}^{t-1} \right) / (1 + \tau),
 $$
остальные пользователи никак не изменяют локальные цены, т.е.  $\underline{\boldsymbol{\lambda}}_{k_t}^t = \underline{\boldsymbol{\lambda}}_{k_t}^{t-1}$.

4. \ev{П}ользователь $k_t$  вычисляет 
$$
x_{k_t}^t(\underline{\lambda}_{k_t,j}^t) = \argmax_{x_k \, \in \, \RR_+} \left (
u_k(x_k) - x_k \sum_{j = 1}^m \underline{\lambda}_{k_t, \, j}^t C_k^j
\right )
$$
и отправляет эту информацию соединениям, которые использует. 

5. \ev{С}оединение $j$ обновля\ev{е}т у себя информацию для $k_t$ пользователя 
$$
y^t_{k_t,j} = b_j - n C_{k_t}^j x_{k_t}(\underline{\boldsymbol{\lambda}}_{k_t}^t).
$$
\ev{Д}анную информацию соединение будет обновлять только 
\ev{в случае, когда через него обменивается пакетами}
пользователь~$k_t$.

\subsection{Оценка скорости сходимости метода экстраполяции случайного градиента}

\ai{В данном разделе мы, \ev{так же, как в} разделе~\ref{fgm}, рассматриваем задачу~\eqref{problem_statement} с $\mu$-сильно вогнутыми функциями затрат $u_k(x_k), \, k = 1, \, \ldots, \, n$. Напомним, что в силу сильной вогнутости функций затрат двойственная задача~\eqref{dual_problem} будет гладкой с константой \ev{Липшица}~$L = \dfrac{nm^2}{\mu}$.}

Для оценки скорости сходимости \ev{метода необходима} следующая оценка для невязки по аргументу из Теоремы~2.1 \cite{lan2018random}:
\begin{equation} \label{th_lan}
    \mathbb{E} \left[\|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^N\|_2^2\right] \leq \frac{4 \Delta \ev{(} \overline{\alpha} \ev{  )} ^N}{\delta},
\end{equation}
где $\Delta = \delta \|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^0\|_2^2 + \frac{B}{n \delta} + \varphi_\delta(\boldsymbol{\lambda}^0) - \varphi_\delta(\boldsymbol{\lambda}^*_\delta)$, $B = ||\mathbf{b}||_2^2$.

Используя \ev{\eqref{th_lan}}, %эту оценку для сходимости по аргументу,
можно \ev{доказать }%сформулировать 
теорему об оценке скорости сходимости метода непосредственно для задачи~\ev{\eqref{regularized}}. 
\begin{theorem}
%\pd{Тут наверное нужно упомянуть, что ситуация аналогична разделу 4: ф-ии $u$ сильно выпуклы и двойственная задача гладкая. Лучше упомянуть, чему равно $L$.}
    Пусть для решения регуляризованной двойственной задачи \eqref{regularized} применяется метод RGEM c параметрами \eqref{params1}, \eqref{params} и $\delta = \frac{\varepsilon}{8 R^2}$ для
    \begin{equation} \label{saga_T1}
 N = \left \lceil 2\left(n + \sqrt{n^2 + \dfrac{128nLR^2}{\varepsilon}}\right)\ln\left(\dfrac{4RA}{\varepsilon} \right) \right \rceil 
    \end{equation}
    итераций, где $A= 2\left( LR + \dfrac{\varepsilon}{8R}\right)\sqrt{6 + \dfrac{16LR^2n + 8B}{n\varepsilon}}$.
% и $B = ||\mathbf{b}||_2^2$. 
Тогда
    $$
    \mathbb{E} \left[U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda}^{N}))\right] \leq \varepsilon, \; \, \, \,  \mathbb{E} \left [ \left \| C \mathbf{x}(\boldsymbol{\lambda}^{N}) - \mathbf{b}\right \|_2\right] \leq \frac{\varepsilon}{2 R}.
    $$
\end{theorem}
%\ev{! В теореме 4 используется C, но у нас это матрица соединений. Просьба заменить на другую букву}
\textbf{Доказательство.} 
%Ввиду сильной выпуклости $\frac{1}{2} %\|\boldsymbol{\lambda}\|_2^2$, имеем
%$$
%P(\boldsymbol{\lambda}^1, \boldsymbol{\lambda}^2) %\geq \frac{1}{2} \|\boldsymbol{\lambda}^2 - %\boldsymbol{\lambda}^1\|_2^2, \quad \forall %\boldsymbol{\lambda}^1, \boldsymbol{\lambda}^2 \in %\Lambda_{2R},
%$$
%Отсюда вместе с \eqref{th_lan} получаем следующую оценку для невязки по аргументу
%\begin{equation} \label{rgem_arg}
 %   \mathbb{E} \left[\|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^N\|_2^2\right] \leq \frac{4 \Delta \overline{\alpha}^N}{\delta}.
%\end{equation}
Из Леммы \ref{lem_regularized_dual} имеем оценки для невязки по ограничениям \eqref{eq_limits_reg1} и по \ev{целевой} функции \eqref{eq_err_reg1}. Ввиду предположения $\boldsymbol{\lambda} \in \Lambda_{2R}$, \ev{выполняются следующие неравенства:}
\begin{equation} \label{ineq_1}
    \|C \mathbf{x}^{N} - \mathbf{b}\|_2 \leq \|\nabla \varphi_\delta (\boldsymbol{\lambda}^{N})\|_2 + 2 \delta R,
\end{equation}
\begin{equation} \label{ineq_2}
    U(\mathbf{x}^{*}) - U(\mathbf{x}^{N}) \leq 2 R \|\nabla \varphi_\delta(\boldsymbol{\lambda}^{N})\|_2 + 4 \delta R^2,
\end{equation}
где  $\mathbf{x}^{N} = \mathbf{x}(\boldsymbol{\lambda}^N)$.
Из Леммы \ref{lem_reqularized_ineqs} и неравенства \eqref{th_lan} получаем следующую оценку для $\|\nabla \varphi_\delta (\boldsymbol{\lambda}^{N})\|_2$\ev{:}
$$
    \mathbb{E} \left[ \|\nabla \varphi_\delta (\boldsymbol{\lambda}^{N})\|_2 \right] \leq 2 (L + \delta) \sqrt{\frac{\Delta}{\delta}} \ev{(}\overline{\alpha}\ev{)}^{N/2}. 
$$
Оценим $\Delta$. \ev{Для функции  $\varphi_\delta$ с липшицевым
градиентом выполняется неравенство 
$$
\varphi_\delta(\boldsymbol{\lambda}^0) - \varphi_\delta(\boldsymbol{\lambda}^*_\delta) \leq \langle \nabla \varphi_{\delta} (\boldsymbol{\lambda}^{*}_\delta), \, \boldsymbol{\lambda}^0 - \boldsymbol{\lambda}^* \rangle + \frac{L + \delta}{2} \|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^0\|_2^2.
$$
}
Учитывая\ev{,} что $\nabla \varphi_{\delta} (\boldsymbol{\lambda}^{*}_\delta)=0$, получаем  
$$
\Delta \leq  \delta \|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^0\|_2^2 + \frac{B}{n \delta} +\frac{L+\delta}{2}\|\boldsymbol{\lambda}^*_\delta - \boldsymbol{\lambda}^0\|_2^2 
\leq (6\delta + 2L)R^2 + \frac{B}{n \delta}.
$$

Пусть $\delta$ подбирается так, чтобы \ev{выполнялось} $4 \delta R^2 = \frac{\varepsilon}{2}$, \ev{тогда} $\delta = \frac{\varepsilon}{8 R^2}$. Отсюда имеем
$$
4 \delta R^2 = \frac{\varepsilon}{2}, \quad 2 \delta R = \frac{\varepsilon}{4 R}.
$$
Потребуем \ev{выполнения неравенства} $U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda}^N)) \leq \varepsilon$. \ev{Тогда, в силу~\eqref{ineq_1}, \eqref{ineq_2} должно выполняться неравенство:}
$$
\|\nabla \varphi_\delta(\boldsymbol{\lambda}^N)\|_2 \leq \frac{\varepsilon}{4 R}.
$$ 
Откуда имеем
$$
2 (L + \delta) \sqrt{\frac{\Delta}{\delta}} \ev{(} \overline{\alpha}\ev{)}^{N/2}  \leq \frac{\varepsilon}{4 R}.
$$
Учитывая, что 
$$
2 (L + \delta) \sqrt{\frac{\Delta}{\delta}}
\ev{\, \leq \, } 2\left( LR + \dfrac{\varepsilon}{8R}\right)\sqrt{6 + \dfrac{16LR^2n + 8B}{n\varepsilon}},
$$
получаем следующую оценку на число итераций 
$$
 N = \left \lceil 2\left(n + \sqrt{n^2 + \dfrac{128nLR^2}{\varepsilon}}\right)\ln\left(\dfrac{4RA}{\varepsilon} \right) \right \rceil,
 $$
 где \ev{$A = 2\left( LR + \dfrac{\varepsilon}{8R}\right)\sqrt{6 + \dfrac{16LR^2n + 8B}{n\varepsilon}}$.}
 $ \quad \blacksquare
 $
 
 
\ai{\textit{Замечание. Отметим, что оценку сложности Алгоритма~\ref{alg_saga} можно также представить в виде $O \left ( \max\left\{n, \, \sqrt{nLR^2/\varepsilon} \right\} \cdot \ln \left( \frac{1}{\varepsilon} \right )\right)$, где логарифмический множитель появляется за сч\ev{ё}т необходимости регуляриз\ev{ации} двойственной задачи. При этом на каждой итерации вычисляется только одна компонента \ev{вектора реакции пользователя на изменение цены, }%градиента, 
соответственно\ev{,} арифметическая сложность операции \ev{лучше, чем при вычислении всех компонент этих векторов. }%маленькая.
\ev{Д}ля БГМ предположения 
\ev{для целевой функции }%{на функцию}
аналогичны, но за сч\ev{ё}т того, что на каждой итерации необходимо вычислять полный градиент\ev{,} стоимость работы алгоритма\ev{,} соответственно\ev{,} %будет
$O\left(n\sqrt{LR^2/\varepsilon} \right)$. Таким образом, несмотря на то\ev{,} что теоретическая оценка скорости сходимости для RGEM имеет тот же порядок\ev{,} что и для БГМ, %\pd{Вроде ведь не хуже. потенциальный выигрыщь корень из $n$}
на практике выигрыш получается за сч\ev{ё}т более деш\ev{ё}вых вычислений в рамках одной итерации.} } 
%\pd{Думаю, стоит пояснить, почему мы рассматриваем этот метод. Предположения для него такие же, как для БГМ. Но хочется получить выигрыш за счет удешевления итерации. Общая стоимость работы алгоритма по идее $n\sqrt{LR^2/\varepsilon}$ для БГМ и $n+\sqrt{nLR^2/\varepsilon}$ для RGEM.}

% \begin{theorem} \label{th_saga_delta}
% 	Пусть для решения регуляризованной двойственной задачи применяется ускоренный метод SAGA с начальной точкой $\lambda_1$, количеством итераций равным $T$, и $\delta = 2 L / 5$. Тогда при $N \leq 2$:
% 	$$
%         \mathbb{E} \left[\|C \mathbf{x}(\boldsymbol{\lambda}_{T}) - \mathbf{b}\|_2\right] \leq D \left(1 + \sqrt{\frac{2}{21 N}}\right)^{-T/2} + \frac{4 L R}{5},
%     $$
%     $$
%         \mathbb{E} \left[U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda}_{T}))\right] \leq 2 R D \left(1 + \sqrt{\frac{2}{21 N}}\right)^{-T/2} + \frac{8 L R^2}{5},
%     $$
%     и при $N > 2$:
%     $$
%         \mathbb{E} \left[\|C \mathbf{x}(\boldsymbol{\lambda}_{T}) - \mathbf{b}\|_2\right] \leq D \left(1 + \frac{1}{2 N}\right)^{-T/2} + \frac{4 L R}{5},
%     $$
%     $$
%         \mathbb{E} \left[U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda}_{T}))\right] \leq 2 R D \left(1 + \frac{1}{2 N}\right)^{-T/2} + \frac{8 L R^2}{5},
%     $$
%     где $\displaystyle D = \frac{84}{5 \sqrt{2}} L R$.
% \end{theorem}
	
% \textbf{Доказательство.} Из Леммы \ref{lem_regularized_dual} имеем оценки для невязки по ограничениям \eqref{eq_limits_reg1} и по функции \eqref{eq_err_reg1}. Ввиду предположения $\lambda \in \Lambda_R$, приходим к
% \begin{equation} \label{th_saga_proof_eq1}
%     \|C \mathbf{x}(\boldsymbol{\lambda}_{T}) - \mathbf{b}\|_2 \leq \|\nabla \varphi_\delta (\boldsymbol{\lambda}_{T})\|_2 + 2 \delta R,
% \end{equation}
% \begin{equation} \label{th_saga_proof_eq2}
%     U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda}_{T})) \leq 2 R \|\nabla \varphi_\delta(\boldsymbol{\lambda}_{T})\|_2 + 4 \delta R^2.
% \end{equation}
% Из Леммы \ref{lem_reqularized_ineqs} и неравенств \eqref{th_zhou_1} и \eqref{th_zhou_2} получаем следующие оценки для $\|\nabla \varphi_\delta (\boldsymbol{\lambda}_{T})\|_2$
% $$
%     \mathbb{E} \left[ \|\nabla \varphi_\delta (\boldsymbol{\lambda}_{T})\|_2 \right] \leq D' \left(1 + \sqrt{\frac{\delta}{3 N (L + \delta)}}\right)^{-T/2} \text{при} \quad \frac{\delta N}{L + \delta} \leq \frac{3}{4}, 
% $$
% $$
%     \mathbb{E} \left[ \|\nabla \varphi_\delta (\boldsymbol{\lambda}_{T})\|_2 \right] \leq D' \left(1 + \frac{1}{2 N}\right)^{-T/2} \qquad \qquad \text{при} \quad \frac{\delta N}{L + \delta} > \frac{3}{4}.
% $$
% где $\displaystyle D' = 4 R (L + \delta) \sqrt{\frac{L}{\delta} + 2}$.
% Откуда и следуют выражения, указанные в формулировке теоремы.
% $$
%     \mathbb{E} \left[\|C \mathbf{x}(\boldsymbol{\lambda}_{T+1}) - b\|_2\right] \leq D' \left(1 + \sqrt{\frac{\delta}{3 N (L + \delta)}}\right)^{-T/2} + 2 \delta R,
% $$
% $$
%     \mathbb{E} \left[f(\mathbf{x}^{*}) - f(\mathbf{x}(\boldsymbol{\lambda}_{T+1}))\right] \leq 2 R D' \left(1 + \sqrt{\frac{\delta}{3 N (L + \delta)}}\right)^{-T/2} + 4 \delta R^2 \qquad \text{при} \quad \frac{\delta N}{L + \delta} \leq \frac{3}{4},
% $$
% и
% $$
%     \mathbb{E} \left[\|C \mathbf{x}(\boldsymbol{\lambda}_{T+1}) - b\|_2\right] \leq D' \left(1 + \frac{1}{2 N}\right)^{-T/2} + 2 \delta R,
% $$
% $$
%     \mathbb{E} \left[f(\mathbf{x}^{*}) - f(\mathbf{x}(\boldsymbol{\lambda}_{T+1}))\right] \leq 2 R D' \left(1 + \frac{1}{2 N}\right)^{-T/2} + 4 \delta R^2 \qquad \text{при} \quad \frac{\delta N}{L + \delta} > \frac{3}{4},
% $$

% Далее, выберем оптимальное значение параметра $\delta$. Для этого требуется решить следующую задачу
% $$
%     \min_\delta \left\{D' = (L+\delta) \sqrt{\frac{L}{\delta} + 2}\right\}.
% $$
% Решим эту задачу явно, приравняв производную этой функции к нулю
% $$
%     \left((L+\delta) \sqrt{\frac{L}{\delta} + 2}\right)' = \sqrt{\frac{L}{\delta}+2} - \frac{L (L+\delta)}{2 \delta^2 \sqrt{\frac{L}{\delta}+2}} = 0 \Rightarrow 
% $$
% $$
%     \Rightarrow \left(\frac{L}{\delta}\right)^2 - \left(\frac{L}{\delta}\right) - 4 = 0 \Rightarrow \frac{L}{\delta} = \frac{1 + \sqrt{17}}{2} \Rightarrow \delta = \frac{2 L}{1 + \sqrt{17}} \approx \frac{2 L}{5}. 
% $$

% Подставляя в неравенства \eqref{th_saga_proof_eq1} и \eqref{th_saga_proof_eq2} оценки для $\|\nabla \varphi_\delta (\boldsymbol{\lambda}_{T})\|_2$ и заменяя в формулах $\delta$ полученным оптимальным значением, приходим к оценкам, указанным в формулировке теоремы. $\quad \blacksquare$




% Регуляризуем двойственную задачу по А.Н. Тихонову:
% $$
%     \varphi(\lambda)_{\delta} = \varphi(\lambda) + \dfrac{\delta}{2}\|\lambda\|^2_2
% $$
% и вместо задачи \eqref{dual_problem} будем решать регуляризованную задачу 
% \begin{equation*}
%     \min_{\lambda \, \in \, \RR_+^m} \varphi_{\delta}(\lambda).
% \end{equation*}
% Параметр $\delta$ будет оптимально подобран позже. 






==> include/conclusion.tex <==
\section{Заключение}


В заключение отметим некоторые возможные развития данной работы и кратко опишем методы без подробного анализа оценки скорости сходимости. 

В параграфе \ref{ellipsoids} мы рассматривали метод эллипсоидов для задач небольшой размерности, который является прямо-двойственным. %Однако 
\ev{С}уществуют и другие методы, которые дают высокую точность и хорошо подходят для задач небольшой размерности. Одним из таких методов является метод Вайды \cite{bubeck}. Однако для восстановления решения прямой задачи при решении двойственной задачи методом Вайды, необходимо  чтобы была сходимость по норме градиента для двойственной задачи. Для этого требуется гладкость двойственной задачи, что порождается сильной выпуклостью 
\ev{целевой функции}
прямой \ev{задачи}~(\ev{У}тверждение~\ref{2_cor_sopr}). Если сильной выпуклости \ev{в} прямой задаче нет, то \ev{её} можно регуляризовать, % прямую задачу 
как %это 
было описано в параграфе~\ref{reg}, но при этом оценка сходимости логарифмически ухудшится. 

Также для решения двойственной задачи можно применить методы высокого порядка \pd{\cite{nesterov2018implementable,gasnikov2019near}}, если двойственная задача достаточно гладкая. \ai{При этом шаги данных методов можно будет считать распределённо}, так как в данной задаче рассматривается централизованная архитектура с точки зрения взаимодействия соединения и использующих его пользователей.  %\pd{, тогда, что? ощущение, что предложение не закончено.}. 
Однако отметим, что оптимальные методы высокого порядка, требующие одномерного поиска и не обладающие прямо-двойственностью, необходимо применять \ev{только после } %предварительно 
регуляризации двойственной задачи. 

Ещ\ev{ё} одно направление\ev{~---} методы типа редукции дисперсии, например, \cite{zhou2018simple, zhou2018direct} которые являются промежуточными между \ev{стохастическим градиентным методом} и \ev{БГМ}. Однако данные методы \ev{тоже} не прямо-двойственные, поэтому их необходимо применять к предварительно регуляризованной двойственной задаче. 

\ev{О}собый интерес для авторов представляют метод Hogwild!~\cite{recht2011hogwild} и методы с использованием мини-батчинга. Заметим, что
\ev{при этом} одновременно данные передают не все пользователи, но и не только один пользователь, как это получается при использовани\ev{и} стохастических методов. \ev{В}ыбирая в качестве размера батча количество пользователей, которые отправляют данные в один момент времени, можно учесть специфику работы реальных сетей. 

%Работа поддержана грантами РФФИ 18-29-03071\_мк и 18-31-20005 мол\_а\_вед, а также грантом Президента РФ МД-1320.2018.1.
Работа в пп.~1-3 поддержана грантом РФФИ 18-29-03071\_мк, в пп.~4-7~--- грантом РФФИ 19-31-51001 Научное наставничество, а в пп.~8-10~---  грантом 18-31-20005 мол\_а\_вед.


==> include/elipsoids.tex <==
\section{Метод эллипсоидов}
\label{ellipsoids}

    В этом параграфе \ev{для решения исходной задачи~\eqref{eq_main_task}
    предлагается применить метод эллипсоидов~\cite{elip_nem}}. Данный метод можно использовать \ev{при} небольшой размерности~\ev{($m$)} двойственной задачи или
    \ev{в случае, когда требуется высокая точность решения}. Данный метод является прямо-двойственным, то есть по решению двойственной задачи можно восстановить решение прямой \ev{задачи}.

    Рассмотрим исходную задачу~\eqref{eq_main_task}
    % $$
    % \max_{\mathbf{x} \geq 0} \left\{ f(\mathbf{x}) = \sum_{i = 1}^N u_i(x^i), C \mathbf{x} \leq b \right\}
    % $$
    и двойственную к ней~\eqref{eq_phi_first}.
    % $$
    % \min_{\boldsymbol{\lambda} \geq 0} \varphi(\boldsymbol{\lambda}), \quad \varphi(\boldsymbol{\lambda}) = \boldsymbol{\lambda} b + \max_{\mathbf{x} \geq 0} \left\{ \sum_{i = 1}^N \left( u_i(x^i) - \boldsymbol{\lambda} C_i x^i \right) \right\},
    % $$
     Как и в предыдущем параграфе, \ev{считаем}, что функции $u_k(x_k)$, $k = 1, \, 
     \ldots, \, n$, являются {\it вогнутыми, но не сильно вогнутыми}. Также предположим, что решение двойственной задачи лежит в евклидовом шаре радиуса~$R$ \ev{с центром в начале координат}, т.е. $\|\boldsymbol{\lambda}^{*}\|_2 \leq  R$.
     В качестве начальной точки метода возьмем нулевой вектор: $\boldsymbol{\lambda}^0 = 0$. Задачу будем решать на множестве:
     $$
    \Lambda_{2R} = \{\boldsymbol{\lambda} \, \in \, \mathbb{R}_{+}^m \, : \, \|\boldsymbol{\lambda}\|_2 \leq 2  R\}.
    $$ 
Привед\ev{ё}м описание метода эллипсоидов (Алгоритм \ref{alg_ellipsoid}), который будем применять для решения двойственной задачи.
    
    \begin{algorithm}
		\caption{Метод эллипсоидов}\label{alg_ellipsoid}
		\begin{algorithmic}[1]
			\Require $u_k(x_k), k = 1, \, \ldots, \, n$~--- вогнутые функции полезностей
			
			\State $B_0 := 2R \cdot I_n$, \ev{$I_n$~--- единичная матрица}
			
			\For{$t=0, \, \ldots, \, N-1$}
    			\State Вычислить $\nabla \varphi(\boldsymbol{\lambda}^t)$
    			
    			\State $\mathbf{q}_t := B_t^T \nabla \varphi(\boldsymbol{\lambda}^t)$
    			\State $\mathbf{p}_t := \displaystyle \frac{B_t^T \mathbf{q}_t}{\sqrt{\mathbf{q}_t^T B_t B_t^T \mathbf{q}_t}}$
    			\State $B_{t+1} := \displaystyle \frac{m}{\sqrt{m^2 - 1}} B_t + \left(\frac{m}{m+1} - \frac{m}{\sqrt{m^2 - 1}}\right) B_t \mathbf{p}_t \mathbf{p}_t^T$
    			\State $\boldsymbol{\lambda}^{t+1} := \boldsymbol{\lambda}^t - \displaystyle \frac{1}{m+1} B_t \mathbf{p}_t$
            \EndFor
			\State\Return $\boldsymbol{\lambda}^N$
		\end{algorithmic}
	\end{algorithm}
	
Для восстановления решения прямой задачи по решению двойственной необходимо определить {\it сертификат точности}~$\xi$ для метода эллипсоидов. Напомним, что сертификатом точности называется последовательность $\xi = \{\xi_t\}_{t=0}^{N-1}$ весов, таких что
	$$
	\xi_t \geq 0, \quad \sum_{t = 0}^{N-1} \xi_t = 1.
	$$
Построение сертификата точности в нашем случае будет осуществляться в процессе работы метода эллипсоидов,
\ev{см. Алгоритм~\ref{alg_cert_ellipsoid}}, общая схема которого такова~\cite{nemirovski2010accuracy}: 
\begin{enumerate}
    \item Находим <<наиболее узкую полоску>>, содержащую эллипсоид~$Q_{N}$, остающийся после итерации $N$, т.e. такой вектор $\mathbf{h}$, что 
    \ev{на $Q_{N}$ выполняется неравенство}:
\begin{equation}
\label{eq_strip}
\max_{\boldsymbol{\lambda} \in Q_{N}} \langle \mathbf{h}, \, \boldsymbol{\lambda} \rangle - \min_{\boldsymbol{\lambda} \in Q_{N}} \langle \mathbf{h}, \, \boldsymbol{\lambda} \rangle \leq 1.
\end{equation}
\ev{Для} метода эллипсоидов \ev{все $Q_N$ представлены как
$$
Q_N = \left \{ B_N \mathbf{z} + \boldsymbol{\lambda}^N : \mathbf{z}^T \mathbf{z} \, \le \, 1 \right \}.
$$
Тогда для решения \eqref{eq_strip} необходимо сделать} сингулярное разложение матрицы $B_{N} = U D V$, где $U$ и $V$~--- ортогональные матрицы и $D$~--- диагональная матрица
\ev{с положительными элементами на диагонали}. Далее искомый вектор~$\mathbf{h}$ определяется следующим образом: $\mathbf{h} = 1/(2 \sigma^{i_*}) \cdot U \mathbf{e}^{i_*}$, где $i_*$~--- индекс наименьшего диагонального элемента матрицы~$D$, $\sigma^{i_*}$~--- соответствующее этому индексу значение элемента матрицы $D$,  $\mathbf{e}^i$~--- векторы стандартного базиса.
    \item Для векторов $\mathbf{h}^{+} = \left [\mathbf{h}, \, -\langle \mathbf{h}, \, \boldsymbol{\lambda}^{N} \rangle \right ]$ и $\mathbf{h}^{-} = -\mathbf{h}^{+}$ находим разложения следующего вида
$$
\mathbf{h}^{+} = \sum_{t=0}^{N-1} \nu_t [\nabla \varphi(\boldsymbol{\lambda}^t), \, -\langle\nabla \varphi(\boldsymbol{\lambda}^t), \,  \boldsymbol{\lambda}^t\rangle] + \mathbf{y}^{+}, \quad 
\mathbf{h}^{-} = \sum_{t=0}^{N-1} \mu_t [\nabla \varphi(\boldsymbol{\lambda}^t), \, -\langle\nabla \varphi(\boldsymbol{\lambda}^t), \, \boldsymbol{\lambda}^t\rangle] + \mathbf{z}^{+},
$$
существование которых следует из утверждения~4.1 \cite{nemirovski2010accuracy}. Этот шаг описывают п.~6--13 рассмотренного ниже \ev{Алгоритма~\ref{alg_cert_ellipsoid}}. 

    \item Из коэффициентов разложения $\nu_t$ и $\mu_t$ векторов $\mathbf{h}^{+}$ и $\mathbf{h}^{-}$, соответственно, получаем выражения для $\xi_t,\; t \in I_{N}$, где $I_{N} = \left\{ t \leq N-1: \, \boldsymbol{\lambda}^t \in \text{\normalfont int}\;\Lambda_{2R} \right\}$. Коэффициенты разложения
    \ev{определяются} только для тех точек, получаемых в процессе работы \ev{Алгоритма~\ref{alg_cert_ellipsoid}}, которые принадлежат допустимому множеству. 
\end{enumerate}
	
	\begin{algorithm}
		\caption{Построение сертификата точности для метода эллипсоидов}\label{alg_cert_ellipsoid}
		\begin{algorithmic}[1]
			\Require $N-1$~--- номер итерации, на которой производится вычисление сертификата точности, $\left\{B_t, \, \boldsymbol{\lambda}^t, \, \nabla \varphi(\boldsymbol{\lambda}^t)\right\}_{t=0}^{N-1}$~--- протокол работы метода эллипсоидов после $N$~итераций
			
			\If{$\nabla \varphi(\boldsymbol{\lambda}^{N-1}) = 0$}
			    \State $\xi_t := 0$ \ev{ для всех } $t = 0, \, \ldots, \, N-2$
			    \State $\xi_{N-1} := 1$
			\Else %If{$\nabla \varphi(\boldsymbol{\lambda}^{N-1}) \neq 0$}
			 %   \State \small Находим "наиболее узкую полоску"\,, содержащую эллипсоид $Q_{T+1}$, остающийся на $T+1$ итерации, то есть такой вектор $\mathbf{h}$, что $\max_{\boldsymbol{\lambda} \in Q_{T+1}} \langle \mathbf{h}, \boldsymbol{\lambda} \rangle - \min_{\boldsymbol{\lambda} \in Q_{T+1}} \langle \mathbf{h}, \boldsymbol{\lambda} \rangle \leq 1$
		        \State \normalsize $\mathbf{h} := 1/(2 \sigma^{i_*}) \cdot U \mathbf{e}^{i_*}$
		      %  \State \small Рассматриваем векторы $\mathbf{h}^{+} = [\mathbf{h}, -\langle \mathbf{h}, \boldsymbol{\lambda}_{T+1} \rangle]$ и $\mathbf{h}^{-} = -\mathbf{h}^{+}$. Найдём их разложения следующего вида
		      %  \noindent $\mathbf{h}^{+} = \sum_{t=1}^T \nu_t [\nabla \varphi(\boldsymbol{\lambda}_t), -\langle\nabla \varphi(\boldsymbol{\lambda}_t), \boldsymbol{\lambda}_t\rangle] + \mathbf{y}^{+},$
		      %  \noindent $\mathbf{h}^{-} = \sum_{t=1}^T \mu_t [\nabla \varphi(\boldsymbol{\lambda}_t), -\langle\nabla \varphi(\boldsymbol{\lambda}_t), \boldsymbol{\lambda}_t\rangle] + \mathbf{z}^{+},$
		      %  существование которых следует из утверждения 4.1 \cite{nemirovski2010accuracy}. 
		        \State \normalsize $\mathbf{g}_\nu := \mathbf{h}, \, \mathbf{g}_\mu := -\mathbf{h}$
		        \For{$t=0, \, \ldots, \, N-1$}
		            \State $\mathbf{q} := B_t^T \nabla \varphi(\boldsymbol{\lambda}^t)$
		            \State $\nu_t := \left[\mathbf{g}_\nu^T B_t \mathbf{q} \right]_{+} / \|\mathbf{q}\|_2^2$
		            \State $\mathbf{g}_\nu := \mathbf{g}_\nu - \nu_t \nabla \varphi(\boldsymbol{\lambda}^t)$
		            \State $\mu_t := \left[\mathbf{g}_\mu^T B_t \mathbf{q}\right]_{+} / \|\mathbf{q}\|_2^2$
		            \State $\mathbf{g}_\mu := \mathbf{g}_\mu - \mu_t \nabla \varphi(\boldsymbol{\lambda}^t)$
		        \EndFor
		        \State \normalsize $\xi_t := (\nu_t + \mu_t) \, / \sum\limits_{i \, \in \, I_{N}} (\nu_i + \mu_i), \quad t \, \in \,  I_{N}$
			\EndIf
			
			\State\Return $\left\{\xi_t\right\}_{t=0}^{N-1}$
		\end{algorithmic}
	\end{algorithm}

% 	\begin{theorem}{\cite{nemirovski2010accuracy}} \label{th_ellipsoid}
% 	Пусть для решения двойственной задачи применяется метод эллипсоидов с начальным шаром $B_0 = \{\boldsymbol{\lambda} \in \mathbb{R}^n: \|\boldsymbol{\lambda}\|_2 \leq 2R\}$ для $T$ итераций, и сертификат точности $\xi$ формируется в соответствии с Алгоритмом \ref{alg_cert_ellipsoid}. Тогда
% 	\begin{equation}\label{th_el-a}
% 	\|[C \hat{\mathbf{x}} - \mathbf{b}]_{+}\|_{2} \leq 32 \cdot 4 M R \exp \left\{ -\frac{T}{2 m (m+1)} \right\},
% 	\end{equation}
% 	\begin{equation}\label{th_el-b}
% 	U(\mathbf{x}^{*}) - U(\hat{\mathbf{x}}) \leq 32 \cdot 4 M R \exp \left\{ -\frac{T}{2 m (m+1)} \right\},
% 	\end{equation}
% % 	где $\displaystyle \hat{\mathbf{x}} = \frac{1}{T} \sum_{t = 1}^T \mathbf{x}(\boldsymbol{\lambda}_t).$
%     где $\displaystyle \hat{\mathbf{x}}_{T} = \sum_{t \in I_{T}} \xi_t \mathbf{x}(\boldsymbol{\lambda}_t), \, \, I_{T} = \left\{ t \leq T: \, \boldsymbol{\lambda}_t \in \text{\normalfont int}\;\Lambda_R \right\}$.
% 	\end{theorem}
Замечание. \textit{Отметим, что, в отличие от БГМ и стохастического \ev{метода проекции субградиента,} в методе эллипсоидов для вычисления шагов~4--6 Алгоритма~\ref{alg_ellipsoid} необходима информация о всех компонентах градиента, \ev{т.е.} нужна информация от всех пользователей. Поэтому необходим общий центр для всех соединений, который будет собирать информацию со всех соединений и выполнять эти вычисления.}
%\subsection{Оценка скорости сходимости метода эллипсоидов}
%\pd{Думаю, что можно не выделять это в отдельную подсекцию.}

Сформулируем теорему об оценк\ev{e} скорости сходимости метода эллипсоидов для решаемой задачи. 	
	\begin{theorem}{\cite{nemirovski2010accuracy}} \label{th_ellipsoid}
	Пусть Алгоритм~\ref{alg_ellipsoid} начинает свою работу
с начальным шаром $B_0 
= \{\boldsymbol{\lambda} \in \mathbb{R}^m: \|\boldsymbol{\lambda}\|_2 \leq 2R\}$ и сертификат точности~$\xi$ формируется в соответствии с Алгоритмом~\ref{alg_cert_ellipsoid}. Тогда после 
	\begin{equation} \label{th_saga}
	    N = 2m(m+1) \ceil[\bigg]{\ln \left(\frac{32 \cdot 4 M R}{\varepsilon}\right)}
	\end{equation}
	итераций будут выполняться следующие неравенства
	$$
    U(\mathbf{x}^{*}) - U(\hat{\mathbf{x}}^N) \leq \varepsilon, \quad \left \|[C \hat{\mathbf{x}}^N - \mathbf{b}]_{+} \right \|_2 \leq \frac{\varepsilon}
    {\evv{R}},
    $$
% 	где $\displaystyle \hat{\mathbf{x}} = \frac{1}{T} \sum_{t = 1}^T \mathbf{x}(\boldsymbol{\lambda}_t).$
    где $\displaystyle \hat{\mathbf{x}}^{N} = \sum_{t \in I_{N}} \xi_t \mathbf{x}(\boldsymbol{\lambda}^t), \quad I_{N} = \left\{ t \leq N-1: \, \boldsymbol{\lambda}^t \in \text{\normalfont int}\;\Lambda_{2R} \right\}$.
	\end{theorem}
Доказательство теоремы можно найти в Приложении. 


==> include/experim.tex <==
\section{Вычислительные эксперименты}
\label{experim}
    \ev{Программный код для} численных экспериментов был написан
    %реализованы 
    на языках программирования Python версии~3.6 и С++ стандарта C++14. Исходный код \ev{для} экспериментов и рассмотренных в статье методов опубликован \ev{на} GitHub и доступен по ссылке: \url{https://github.com/dmivilensky/network-resource-allocation}\ev{.} 

    \subsection{Сети с двумя соединениями и квадратичными \ev{функциями} полезности}
    Рассмотрим задачу \eqref{eq_main_task} для сети с двумя соединениями с одинаковыми пропускными способностями (вектор $\mathbf{b} = (5, \, 5)$), используемыми одновременно большим числом пользователей ($n = 1.5 \cdot 10^3$, $C\ev{_{i}^j} = 1,\;\; \forall \, i, \, j$). Функции полезностей имеют вид
    $$
        u_k(x_k) = a_k x_k - \frac{\sigma n}{2} x_k^2, \quad a_k \sim U([0, \, 100])\text{~--- н.о.р}\;, \sigma=0.1.
    $$
    Тогда задачу \eqref{eq_xi_argmax} можно решить явно
    $$
    \mathbf{x}(\mathbf{\lambda}) = \frac{[\mathbf{a} - C \boldsymbol{\lambda}]_{+}}{n \sigma}.
    $$

    Применим для решения двойственной задачи быстрый градиентный метод (алгоритм \ref{alg_fgm}) с начальной ценой $\boldsymbol{\lambda} = \mathbf{0}$. Решение было найдено за 350 итераций метода. При применении метода экстраполяции случайного градиента (алгоритм \ref{alg_saga}) решение задачи было найдено за 3000 итераций. Изменение невязки по ограничениям и зазора двойственности в процессе работы методов показано на рис. 2, (a)-(b) (для логарифмической шкалы числа итераций). 
    
    Несмотря на большее число итераций метода экстраполяции случайного градиента по сравнению с БГМ,%, например, с быстрым градиентным методом,
    для $n \gg 0$ число требующихся запросов оптимального решения $x_k(\boldsymbol{\lambda})$ от пользователей будет меньшим, чем при использовании других алгоритмов. В данном эксперименте 
    %$n = 1.5 \cdot 10^3, T_{FGM} = 350, T_{SSM} = 3000$, 
    за одну итерацию метода экстраполяции случайного градиента запрос отправляется только к одному случайному пользователю и суммарное число запросов будет равно $3000$, тогда как \ev{БГМ} потребуется вычисление всех компонент вектора $\mathbf{x}(\lambda)$, \ev{т.е.} необходимо будет отправить $5.25 \cdot 10^5$ запросов.
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/7-Cb-q-m=2,n=1500.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/8-Uphi-q-m=2,n=1500.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость быстрого градиентного метода (алгоритм \ref{alg_fgm}) и метода экстраполяции случайного градиента (алгоритм \ref{alg_saga}) к решению для сети с двумя соединениями  и квадратичными \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}
    
    \subsection{Сети с двумя соединениями и логарифмическими \ev{функциями} полезности}
    Рассмотрим работу стохастического субградиентного метода (алгоритм \ref{alg_stoch}) и метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) для сети, аналогичной описанной в предыдущем разделе.
    \ev{Число пользователей} $n = 1.5 \cdot 10^3$ с равномерным спросом на ресурсы сети ($C\ev{_{i}^j} = 1,\;\; \forall \, i, \, j$).
    Функции полезности следующего вида:
    $$
        u_k(x_k) = \ln{x_k}.
    $$
    В таком случае явное решение задачи \eqref{eq_xi_argmax} выглядит следующим образом (операция $1 / \cdot$ применительно к вектору понимается поэлементно)\ev{:}
    $$
        \mathbf{x}(\boldsymbol{\lambda}) = \frac{1}{C \boldsymbol{\lambda}}.
    $$
    
    При использовании стохастического субградиентного метода с начальным значением цен $\boldsymbol{\lambda} = (1, \, 1)$, решение было получено за 2000 итераций. 
    \ev{При применении }%Используя 
    метода эллипсоидов с начальным шаром радиуса~$R = 100$ для %решения 
    двойственной задачи, решение %задачи 
    было найдено за 40 итераций. Сходимость методов \ev{к решению } показана на рис. 3, (a)-(b).
    
    Отметим, что аналогично %случаю 
    метод\ev{у} экстраполяции случайного градиента, стохастический субградиентный метод требует вычисления лишь одной компоненты вектора $\mathbf{x}(\boldsymbol{\lambda})$ реакций пользователей на установившиеся цены на каждой итерации. Таким образом, при большем числе итераций метода число вычисляемых компонент $x_k(\boldsymbol{\lambda}^t)$ будет меньшим по сравнению с другими алгоритмами, например, \ev{с} методом эллипсоидов, также как и коммуникационная сложность в случае распределённой реализации.
    
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/1-Cb-log-m=2,n=1500.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/2-Uphi-log-m=2,n=1500.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) и стохастического субградиентного метода (алгоритм \ref{alg_stoch}) к решению для сети с двумя соединениями  и логарифмическими \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}
    
    \subsection{Сети с пятью соединениями и квадратичными \ev{функциями} полезности}
    Рассмотрим работу методов для сети с числом соединений $5$. Пусть число пользователей $n = 1.5 \cdot 10^3$, функции полезности для каждого из пользователей квадратичны, пропускные способности каждого из соединений $b_j$ выбираются равновероятно из отрезка $[1, \, 6]$, а матрица спроса на ресурсы сети $C$ заполняется случайно, т.е. для любых $i$, $j$ с вероятностью $p=0.5$ пользователю $i$ требуется соединение $j$ и $C\ev{_{i}^j} = 1$, а с вероятностью $p=0.5$~--- $C\ev{_{i}^j} = 0$.
    
    При использовании \ev{БГМ} (алгоритм \ref{alg_fgm}) для получения решения задачи потребовалось 380~итераций. \ev{При применении }%Используя 
    метода экстраполяции случайного градиента~(алгоритм \ref{alg_saga}), решение задачи было найдено за 6700~итераций. Сходимость методов \ev{к решению} показана на рис. 4, (a)-(b).
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/9-Cb-q-m=5,n=1500.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/10-Uphi-q-m=5,n=1500.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость быстрого градиентного метода (алгоритм \ref{alg_fgm}) и метода экстраполяции случайного градиента (алгоритм \ref{alg_saga}) к решению для сети с пятью соединениями  и квадратичными \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}
    
    \subsection{Сети с пятью соединениями и логарифмическими \ev{функциями} полезности}
    Рассмотрим работу методов для сети \ev{с} пятью соединениями, структура которой аналогична приведённой выше, и логарифмиче\ev{с}ких функций полезности.
    
    При использовании стохастического субградиентного метода (алгоритм \ref{alg_stoch}) из начального значения $\boldsymbol{\lambda} = (0.1, \, 0.1, \, 0.1, \, 0.1, \, 0.1)$ решение было получено за 2500 итераций. \ev{При применении }%Используя 
    метода эллипсоидов~(алгоритм \ref{alg_ellipsoid}) с начальным шаром радиуса $R = 4$ решение двойственной задачи было получено за 85 итераций. Сходимость методов \ev{к решению} показана на рис. 5, (a)-(b).
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/3-Cb-log-m=5,n=1500.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/4-Uphi-log-m=5,n=1500.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) и стохастического субградиентного метода (алгоритм \ref{alg_stoch}) к решению для сети с пятью соединениями  и логарифмическими
    \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}
    
    \subsection{Сети с большим числом соединений и квадратичными \ev{функциями} полезности}
    Применим быстрый градиентный метод (алгоритм \ref{alg_fgm}) и метод экстраполяции случайного градиента (алгоритм \ref{alg_saga}) к сети с более сложной структурой. Рассмотрим случай $n=5 \cdot 10^3$ и $m=70$, где $n$~--- число пользователей и $m$~--- число соединений в сети. Матрица $C$ спроса пользователей заполняется случайно, значения компонент вектора пропускных способностей $\mathbf{b}$ выбираются равновероятно из отрезка $[1, \, 6]$. 
    
    При использовании \ev{БГМ} для указанной конфигурации сети решение было получено за 400 итераций. При применении метода экстраполяции случайного градиента для получения решения потребовалось 7800 итераций. Сходимость методов показана на рис. 6, (a)-(b).
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/11-Cb-q-m=70,n=5000.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/12-Uphi-q-m=70,n=5000.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость быстрого градиентного метода (алгоритм \ref{alg_fgm}) и метода экстраполяции случайного градиента (алгоритм~\ref{alg_saga}) к решению для сети с 70 соединениями  и квадратичными \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}
    
    \subsection{Сеть с большим числом соединений и логарифмическими \ev{функциями} полезности}
    При использовании стохастического субградиентного метода (алгоритм~\ref{alg_stoch}) для сети из $m = 70$ соединений со случайно распределённым спросом пользователей ($n = 5 \cdot 10^5$) решение задачи было получено за 4000~итераций. 
    \ev{При применении }%Применяя 
    метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) с начальным шаром радиуса $R = 400$ решение было получено за 120 итераций. Сходимость методов показана на рис.~7, (a)-(b).
    
    \begin{figure}
    \centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/5-Cb-log-m=70,n=5000.png}
        \caption{}
        \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{include/plots/6-Uphi-log-m=70,n=5000.png}
        \caption{}
        \end{subfigure}
    \caption{Сходимость метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) и стохастического субградиентного метода (алгоритм \ref{alg_stoch}) к решению для сети с 70 соединениями  и логарифмическими \ev{функциями} полезности: (a) невязка по ограничениям; (b) зазор двойственности}
    \end{figure}

==> include/experim_new.tex <==
\section{Вычислительные эксперименты}
\label{experim}
    Программный код для численных экспериментов был написан на языках программирования Python версии~3.6 и С++ стандарта C++14. Исходный код для экспериментов и рассмотренных в статье методов опубликован на GitHub и доступен по ссылке: \url{https://github.com/dmivilensky/network-resource-allocation}. Измерение времени работы производилось на компьютере с 2-ядерным процессором Intel Core i5-5250U с тактовой частотой 1,6 ГГц на каждое ядро, ОЗУ компьютера составляла 8 Гб.

    \subsection{Сильно выпуклые (квадратичные) функции полезности}
    Рассмотрим задачу \eqref{eq_main_task} для функций полезности следующего вида
    $$
        u_k(x_k) = a_k x_k - \frac{\sigma n}{2} x_k^2, \quad a_k \sim \mathcal{U}(0, \, 100)\text{~--- н.о.р }\;, \sigma=0.1.
    $$
    Тогда задачу \eqref{eq_xi_argmax} можно решить явно:
    $$
    \mathbf{x}(\mathbf{\lambda}) = \frac{[\mathbf{a} - C \boldsymbol{\lambda}]_{+}}{n \sigma}.
    $$
    
    Для малого числа пользователей ($n=1500$) пропускные способности соединений выбираются одинаковыми (в данном случае $\mathbf{b} = (5, \, \ldots, \, 5)^\top$), а спрос на передачу информации равномерен ($c_{i j} = 1$ для любых $i, \, j$). Для большего числа пользователей вектор пропускных способностей генерируется случайно, так что $b_i \sim \mathcal{U}(1, 6)$. Также случайно и независимо выбираются элементы матрицы спроса, так что $c_{i j} = 1$ с вероятностью $p = 0.5$ и $c_{i j} = 0$ с вероятностью $q = 0.5$.
    
    В таблице~\ref{table_quadratic} представлены число итераций и время работы быстрого градиентного метода (FGM) и метода экстраполяции случайного градиента (RGEM) для различных конфигураций сети (с числом соединений $m$), числа пользователей $n$ и требуемой точности $\varepsilon$. В таблице выделены те случаи, в которых метод экстраполяции случайного градиента сходится к решению за меньшее время, чем быстрый градиентный метод, несмотря на большее число итераций по сравнению с БГМ. Действительно, для $n \gg 0$ число требующихся запросов оптимального решения $x_k(\boldsymbol{\lambda})$ от пользователей, в случае метода экстраполяции случайного градиента, будет меньшим, чем при использовании других алгоритмов, так как за одну итерацию метода экстраполяции случайного градиента запрос отправляется только к одному случайному пользователю.
    
    \begin{table}[h]
    \begin{center}
\begin{tabularx}{1\textwidth}{|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2.9cm}|>{\centering\arraybackslash}m{2.8cm}|>{\centering\arraybackslash}m{2.9cm}|>{\centering\arraybackslash}m{2.8cm}|}
    \hline
    & \multicolumn{2}{c}{FGM} & \multicolumn{2}{|c|}{RGEM} \\
    \hline
    Сеть & Число итераций & Время работы & Число итераций & Время работы \\ 
    \hline
    \hline
    $m~=~2$ $n~=~1500$ $\varepsilon~=~10^{-2}$ & \textbf{350} & \textcolor{blue}{\textbf{24,5} с} & \textbf{3000} & \textcolor{blue}{\textbf{21,1} с} \\
    \hline
    $m~=~5$ $n~=~1500$ $\varepsilon~=~10^{-2}$ & \textbf{380} & \textcolor{blue}{\textbf{42,7} с} & \textbf{6700} & \textcolor{blue}{\textbf{36,9} с} \\ 
    \hline
    $m~=~70$ $n~=~5000$ $\varepsilon~=~10^{-2}$ & \textbf{400} & \textcolor{blue}{\textbf{150,0} с} & \textbf{7800} & \textcolor{blue}{\textbf{132,6} с} \\
    \hline
    $m~=~70$ $n~=~5000$ $\varepsilon~=~10^{-3}$ & \textbf{1070} & \textcolor{blue}{\textbf{374,5} с} & \textbf{9180} & \textcolor{blue}{\textbf{283,7} с} \\ 
    \hline
    $m~=~100$ $n~=~5000$ $\varepsilon~=~10^{-2}$ & \textbf{417} & \textcolor{blue}{\textbf{175,1} с} & \textbf{8200} & \textcolor{blue}{\textbf{164,0} с} \\
    \hline
    $m~=~70$ $n~=~7000$ $\varepsilon~=~10^{-2}$ & \textbf{421} & \textcolor{blue}{\textbf{218,9} с} & \textbf{8600} & \textcolor{blue}{\textbf{206,4} с} \\ 
    \hline
    $m~=~100$ $n~=~7000$ $\varepsilon~=~10^{-2}$ & \textbf{427} & \textcolor{blue}{\textbf{290,3} с} & \textbf{9200} & \textcolor{blue}{\textbf{276,0} с} \\
    \hline
    $m~=~100$ $n~=~7000$ $\varepsilon~=~10^{-3}$ & \textbf{1120} & \textcolor{blue}{\textbf{761,6} с} & \textbf{10130} & \textcolor{blue}{\textbf{638,2} с} \\ 
    \hline
\end{tabularx}
\end{center}
    \caption{Сравнение количества итераций и времени работы БГМ и метода экстраполяции случайного градиента для сильно выпуклых (квадратичных) функций полезности}
    \label{table_quadratic}
\end{table}
    
    \subsection{Выпуклые (логарифмические) функции полезности}
    Рассмотрим работу стохастического субградиентного метода (алгоритм \ref{alg_stoch}) и метода эллипсоидов (алгоритм \ref{alg_ellipsoid}) для функции полезности следующего вида:
    $$
        u_k(x_k) = \ln{x_k}.
    $$
    В таком случае явное решение задачи \eqref{eq_xi_argmax} выглядит следующим образом (операция $1 / \cdot$ применительно к вектору понимается поэлементно)\ev{:}
    $$
        \mathbf{x}(\boldsymbol{\lambda}) = \frac{1}{C \boldsymbol{\lambda}}.
    $$
    
    Для малого числа пользователей ($n=1500$) пропускные способности соединений выбираются одинаковыми (в данном случае $\mathbf{b} = (5, \,\
    \ldots, \,5)^\top$), а спрос на передачу информации равномерен ($c_{i j} = 1$ для любых $i, \, j$). Для большего числа пользователей вектор пропускных способностей генерируется случайно, так что $b_i \sim \mathcal{U}(1, 6)$. Также случайно и независимо выбираются элементы матрицы спроса, так что $c_{i j} = 1$ с вероятностью $p = 0.5$ и $c_{i j} = 0$ с вероятностью $q = 0.5$.
    
    В таблице~\ref{table_log} представлены число итераций и время работы стохастического субградиентного метода (SGM) и метода эллипсоидов для различных конфигураций сети, числа пользователей и требуемой точности. В таблице выделены те случаи, в которых стохастический субградиентный метод сходится к решению за меньшее время, чем метод эллипсоидов.
    
    Отметим, что аналогично
    методу экстраполяции случайного градиента, стохастический субградиентный метод требует вычисления лишь одной компоненты вектора $\mathbf{x}(\boldsymbol{\lambda})$ реакций пользователей на установившиеся цены на каждой итерации. Таким образом, при большем числе итераций метода число вычисляемых компонент $x_k(\boldsymbol{\lambda}^t)$ будет меньшим по сравнению с другими алгоритмами, например, с методом эллипсоидов, также как и коммуникационная сложность в случае распределённой реализации.
    
    \begin{table}[h]
    \begin{center}
\begin{tabularx}{1\textwidth}{|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2.9cm}|>{\centering\arraybackslash}m{2.8cm}|>{\centering\arraybackslash}m{2.9cm}|>{\centering\arraybackslash}m{2.8cm}|}
    \hline
     & \multicolumn{2}{c}{Метод эллипсоидов} & \multicolumn{2}{|c|}{SGM} \\
    \hline
    Сеть & Число итераций & Время работы & Число итераций & Время работы \\ 
    \hline
    \hline
    $m~=~2$ $n~=~1500$ $\varepsilon~=~10^{-2}$&  \textbf{40} & \textbf{0,02} с & \textbf{2000} & \textbf{0,2} с\\
    \hline
    $m~=~5$ $n~=~1500$ $\varepsilon~=~10^{-2}$&  \textbf{85} & \textbf{0,06} с & \textbf{2500} & \textbf{0,3} с\\ 
    \hline
    $m~=~70$ $n~=~5000$ $\varepsilon~=~10^{-2}$&  \textbf{120} & \textcolor{blue}{\textbf{1,9} с} & \textbf{4000} & \textcolor{blue}{\textbf{1,3} с}\\
    \hline
    $m~=~70$ $n~=~5000$ $\varepsilon~=~10^{-3}$&  \textbf{800} & \textcolor{blue}{\textbf{5,4} с} & \textbf{9020} & \textcolor{blue}{\textbf{2,4} с}\\ 
    \hline
    $m~=~100$ $n~=~5000$ $\varepsilon~=~10^{-2}$&  \textbf{300} & \textcolor{blue}{\textbf{9,0} с} & \textbf{5000} & \textcolor{blue}{\textbf{3,1} с}\\
    \hline
    $m~=~70$ $n~=~7000$ $\varepsilon~=~10^{-2}$&  \textbf{250} & \textcolor{blue}{\textbf{8,7} с} & \textbf{5590} & \textcolor{blue}{\textbf{5,5} с}\\ 
    \hline
    $m~=~100$ $n~=~7000$ $\varepsilon~=~10^{-2}$&  \textbf{380} & \textcolor{blue}{\textbf{19,0} с} & \textbf{6480} & \textcolor{blue}{\textbf{10,8} с} \\
    \hline
    $m~=~100$ $n~=~7000$ $\varepsilon~=~10^{-3}$&  \textbf{1830} & \textcolor{blue}{\textbf{91,5} с} & \textbf{17970} & \textcolor{blue}{\textbf{30,6} с} \\ 
    \hline
\end{tabularx}
\end{center}
    \caption{Сравнение количества итераций и времени работы стохастического субградиентного метода и метода эллипсоидов для выпуклых (логарифмических) функций полезности}
    \label{table_log}
\end{table}

==> include/fgm.tex <==
\section{Быстрый градиентный метод}\label{fgm}
В данном разделе мы предполагаем, что
функции полезности $u_k(x_k)$, $k = 1, \, \ldots, \, n$, являются {\it сильно вогнутыми} с константой~$\mu$, следовательно,
двойственная задача будет гладкой. 

Для решения двойственной задачи~\eqref{dual_problem} применим быстрый градиентный метод (БГМ) Нестерова 
в следующем варианте
(метод PDFGM, см. Алгоритм~\ref{alg_fgm}). 
%\floatname{algorithm}{Алгоритм}
	\begin{algorithm}
		\caption{Прямо-двойственный быстрый градиентный метод (PDFGM)}\label{alg_fgm}
		\begin{algorithmic}[1]
			
			\Require $u_k(\mathbf{x}), \; \; k=1, \, \ldots, \, n$~--- сильно вогнутые функции полезности для каждого пользователя; $\boldsymbol{\lambda}^{0}$~--- вектор начальных цен, $\alpha_{t}: = \frac{t+1}{2}$, 
			\evv{$A_{-1} := 0$, } 
			$A_t := A_{t-1} + \alpha_{t} = \frac{(t+1)(t+2)}{4}$, $\tau_{t}: = \frac{\alpha_{t+1}}{A_{t+1}}=\frac{2}{t + 3}$, \evv{$t = 0, \, 1, \, \ldots, \, N-1$}.	

			%\Ensure цена $p^N$, для которой выполняется $\left|C-\sum \limits_{k=1}^n x_k(p^N)\right|\leqslant   \varepsilon$.
			\For{$t=0,\, 1, \, \ldots, \, N-1$}
			\State Вычислить $\varphi(\boldsymbol{\lambda}^t)$, $\nabla \varphi(\boldsymbol{\lambda}^t)$ 
			\State $\mathbf{y}^t :=
\left [ 
\boldsymbol{\lambda}^t - \frac{1}{L}
\left (
\mathbf{b} - \sum\limits_{k = 1}^n \mathbf{C}_k x_k (\boldsymbol{\lambda}^t)
\right )
\right ]_+$			
			%\argmin\limits_{\boldsymbol{\lambda} %\, \in \, \RR_+^m} \left \{ %\varphi(\boldsymbol{\lambda}^t) + %\nabla \varphi %(\boldsymbol{\lambda}^t) %(\boldsymbol{\lambda} - %\boldsymbol{\lambda}^t) + \frac{L}{2} %\| \boldsymbol{\lambda} - %\boldsymbol{\lambda}^t \|_2^2 
			%\right
			%\}$
			\State $\mathbf{z}^t := 
				\left[
				\boldsymbol{\lambda}^0 - \frac{1}{L}
		\sum\limits_{j=0}^t \alpha_j
\left (
\mathbf{b} - \sum\limits_{k = 1}^n \mathbf{C}_k x_k^{\evv{}} (\boldsymbol{\lambda}^{\evv{j}})
\right )
		\right]_{+}.
			$
			%\argmin\limits_{\boldsymbol{\lambda} \, \in \, \RR_+^m} \left \{
		%	\frac{L}{2} \| \boldsymbol{\lambda} - \boldsymbol{\lambda}^0 \|_2^2 +
	%		\sum\limits_{j = 0}^t \alpha_j
	%		%\left [ 
	%		 			\nabla \varphi (\boldsymbol{\lambda}^j) (\boldsymbol{\lambda} - \boldsymbol{\lambda}^j) 
	%		 			%\right ] 
	%		\right
	%		\}$
			
			\State $\boldsymbol{\lambda}^{t + 1} := \tau_t \mathbf{z}^t + (1 - \tau_t) \mathbf{y}^t$
			
			\State $\mathbf{\hat{x}}^{t+1} := \frac{1}{A_{t+1}}
			\sum\limits_{j=0}^{t+1} \alpha_j \mathbf{x}(\boldsymbol{\lambda^{j}})$
\EndFor
			\State\Return $\boldsymbol{\lambda}^{N}$, $\mathbf{\hat{x}}^{N}$
		\end{algorithmic}
	\end{algorithm}

\subsection{Распределённый метод}
Для решения рассматриваемой задачи
можно также применить БГМ в распределённом варианте, что означает, что каждое соединение может вычислять оптимальную скорость передачи данных только исходя из реакции пользователей, которые используют данное соединение, и никак не взаимодействовать с другими соединениями. 

Опишем процесс, происходящий на $t$-ой итерации для соединения $j$:

1. На основе информации, полученной
от пользователей
после предыдущей итерации с номером~$t-1$  (вектор $\mathbf{x}^t=\mathbf{x}(\boldsymbol{\lambda}^t)$), соединение $j$ вычисляет 
$$
y_{j}^t = \left[\lambda_{j}^t -
			\frac{1}{L}
			\left ( b_j - \sum\limits_{k = 1}^n C_k^j x_k^t \right )\right]_{+}.
			$$
При этом $C_k^j \neq 0$ только для тех пользователей, которые используют соединение~$j$. Поэтому для вычисления этого шага соединению нужна только информация от пользователей, которые используют это соединение. 

2. Далее соединение $j$ аналогично вычисляет 
$$z_{j}^t = 
			\left[\lambda_j^0 - \frac{ \alpha_j}{L}
		\left ( b_j - \sum\limits_{k = 1}^n C_k^j  {x}_k^t \right )\right]_{+}.	
			$$
			
3. Получив значения на предыдущих двух шагах, соединение~$j$ вычисляет цену 
для следующей итерации~$t+1$:
$$\lambda^{t + 1}_j = \tau_t z_j^t + (1 - \tau_t) y_j^t$$
и посылает эту информацию всем пользователям, которые с ним соединены.

4. Далее пользователи вычисляют оптимальные скорости передачи
информации $\mathbf{\hat{x}}^{t+1}$, в частности, для пользователя~$k$ получаем 
$$
x_k(\boldsymbol{\lambda}^{t+1}) = \argmax_{x_k \, \in \, \RR_+} \left (
u_k(x_k) - x_k \sum_{j = 1}^m \lambda^{t+1}_j C_k^j
\right ),
$$
где в силу определения матрицы~$C$ пользователю необходима информация только от соединений, которые он использует. Далее пользователь вычисляет оптимальную скорость
$$
\hat{x}^{t+1}_k = \frac{A_{t} \hat{x}^{t}_k + x^{t+1}_k}{A_{t+1}}.
$$

Замечание. \textit{Минусом данного алгоритма является то, что каждому соединению необходимо знать реакции всех пользователей, которые его используют на каждой итерации. К сожалению, в реальных сетях пользователи отправляют данные неодновременно, поэтому достаточно сложно собрать данную информацию для соединения. Однако наличие полной информации о пользователях позволяет соединению быстрее устанавливать равновесную цену.}

\subsection{Оценка скорости сходимости БГМ}
Прежде чем привести доказательство
сходимости БГМ для рассматриваемой задачи, сформулируем ключевую лемму, необходимую для получения оценок невязки в ограничениях и зазора двойственности после
работы прямо-двойственного метода~PDFGM. 
\begin{Lem}
\label{lem_est_1}
Пусть Алгоритм~\ref{alg_fgm} начинает свою работу
с начальной точки $\boldsymbol{\lambda}^0$, 
которая лежит в евклидовом шаре радиуса~$R$ с центром в начале координат. Тогда после $N$ итераций Алгоритма~\ref{alg_fgm} будет
выполняться следующее неравенство:
\begin{equation}
\label{eq_aur37}
A_N \varphi(\mathbf{y}^N) - A_N U(\mathbf{\hat{x}}^{N})
+ 2 \hat R A_N \left \|\left ( C \mathbf{\hat{x}}^N - \mathbf{b} \right )_+ \right \|_2 \, \le \,\frac{ 37L\hat R^2}{9}.
\end{equation}
где $\mathbf{\hat{x}}^N = \frac{1}{A_N}
\sum\limits_{t = 0}^{N-1} \alpha_t \mathbf{x}(\boldsymbol{\lambda}^t)$  и $\hat R = 3R$.
\end{Lem}
Доказательство леммы можно найти в Приложении. 

Теперь сформулируем теорему об оценке скорости сходимости Алгоритма~\ref{alg_fgm}.
\begin{theorem}
\label{main_th_fgm}
Пусть Алгоритм~\ref{alg_fgm} начинает свою работу
с начальной точки $\boldsymbol{\lambda}^0$,
которая лежат в евклидовом шаре радиуса~$R$ {с центром в начале координат}.
Тогда после
\begin{equation}
\label{eq_fgm_t_iter}
N = \left \lceil \frac{2 \hat{R}}{3}\sqrt{\frac{37 L}{\varepsilon}} \right \rceil    
\end{equation}
итераций Алгоритма~\ref{alg_fgm} будут
выполняться следующие неравенства:
\begin{equation*}
U(\mathbf{x^*}) - U(\mathbf{\hat{x}}^{N}) \,  \le \, \varepsilon, \, \, \, \, 
  \left \| \left (C \mathbf{\hat{x}}^N - \mathbf{b} \right)_{+}\right \|_2 \, \le \, \frac{\varepsilon}{\hat R},
\end{equation*}
где $\mathbf{\hat{x}}^N = \frac{1}{A_N}
\sum\limits_{t = 0}^{N-1} \alpha_t \mathbf{x}(\boldsymbol{\lambda}^t)$, 
$\mathbf{x^*}$ ~--- оптимальное решение задачи~\eqref{eq_main_task},
$\hat R = 3R$.
\end{theorem}
\textbf{Доказательство.}
Обозначим оптимальное значение исходной прямой задачи~\eqref{eq_main_task} $Opt[P]$,
а оптимальное значение двойственной задачи~\eqref{dual_problem}~--- $Opt[D]$.
В силу слабой двойственности
\begin{equation*}
\label{eq_dp}
Opt[D] \, \ge \, Opt[P].    
\end{equation*}
Кроме того,
для всех $\mathbf{x} \, \in \, \mathbb{R}^n_+$
и оптимального решения двойственной задачи~\eqref{dual_problem} $\boldsymbol{\lambda^*}$
\begin{equation}
\label{eq_optpu}
Opt[P] \, \ge \, U(\mathbf{x}) - 
\langle 
\boldsymbol{\lambda^*}, \,
\left ( \sum_{k = 1}^n \mathbf{C}_k x_k  - \mathbf{b}  \right )_+
 \rangle \geq U(\mathbf{x}) - \hat R \left \| \left ( C \mathbf{x} - \mathbf{b}   \right)_{+}\right \|_2.
\end{equation}
Тогда
\begin{eqnarray*}
\varphi(\mathbf{y}^N) -  U(\mathbf{\hat{x}}^{N}) & =& \varphi(\mathbf{y}^N) -  U(\mathbf{\hat{x}}^{N}) + Opt[P] - Opt[P]
+ Opt[D] - Opt[D] = \\ &
= & \underbrace{\left (Opt[D] - Opt[P] \right )}_{\geq 0}+
\left (Opt[P] - U(\mathbf{\hat{x}}^{N}) \right ) +
\underbrace{\left (\varphi(\mathbf{y}^N) - Opt[D] \right )}_{\geq 0} \, \\ & \overset{\eqref{eq_optpu}}{\ge} &\, 
- \langle \boldsymbol{\lambda^*}, \, \left ( \mathbf{b} - C \mathbf{\hat{x}}^N \right )_+ \rangle 
\, \ge 
- \hat R \left \| \left ( C \mathbf{\hat{x}}^N - \mathbf{b} \right)_{+}\right \|_2.
\end{eqnarray*}
После подстановки последнего неравенства
в~\eqref{eq_aur37} получим следующую оценку 
\begin{equation*}
 \label{eq_fgm_r37}
 \hat R \left \| \left( C \mathbf{\hat{x}}^N - \mathbf{b}\right)_{+}\right \|_2 \, \le \frac{37 L\hat R^2}{9A_N}.
\end{equation*}
Следовательно,
$\varphi(\mathbf{y}^N) -  U(\mathbf{\hat{x}}^{N}) \, \ge \, -\frac{37 L\hat R^2}{9A_N}$.
С другой стороны, из~\eqref{eq_aur37} следует,
что
$\varphi(\mathbf{y}^N) -  U(\mathbf{\hat{x}}^N) \, \le \, \frac{37 L\hat R^2}{9A_N}$.
Поэтому
$$
\left | \varphi(\mathbf{y}^N) -  U(\mathbf{\hat{x}}^{N}) \right | \, \le \, \frac{37 L\hat R^2}{9A_N}.
$$
Так как $\varphi(\mathbf{y}^N) \, \ge \, Opt[D] = \varphi(\mathbf{y^*}) 
\, \ge \, Opt[P] = U(\mathbf{x^*})$,
выполняется следующее неравенство
\begin{equation*}
\label{eq_uu148}
U(\mathbf{x^*}) - U(\mathbf{\hat{x}}^{N}) \, \le \, \frac{37 L\hat R^2}{9A_N} = \frac{148 L\hat R^2}{9(N+1)(N+2)} \leq \frac{148 L\hat R^2}{9N^2} \leq \varepsilon.
\end{equation*}
Выражая из последнего неравенства $N$, получаем оценку из условия теоремы. $\blacksquare$


%-----------------------------------------


















==> include/intro.tex <==
\section{Введение}
\subsection{Мотивация}
В этой статье мы рассматриваем задачу управления  современными сетями связи с точки зрения оптимизации и стохастического моделирования. Для решения задач такого рода
необходимо представить
и проанализировать математическую модель, возникающую при симуляции
процесса работы крупномасштабных широкополосных сетей. Ожидается, что в будущих сетях связи появятся приложения, которые смогут изменять свои скорости передачи данных в соответствии с доступной пропускной способностью в сети. В качестве примера такой сети можно привести TCP-трафик через сеть Интернет. 

Ключевой вопрос, который мы рассматриваем в этой статье, касается того, как доступная пропускная способность в сети должна быть распределена между конкурирующими потоками. При этом 
контроль над использованием потребителями доступных пропускных способностей осуществляется посредством корректировки цены на соединение. 

Таким образом, в работе рассматривается задача
оптимизации распределения ресурсов в компьютерных сетях с большим числом соединений.
Соединения используют для своих целей
потребители (пользователи), число которых
также может быть очень большим. 
Цель работы состоит в определении механизма управления ресурсами, которые в контексте данной задачи являются доступными пропускными способностями соединений. При этом необходимо обеспечить стабильную работу системы и предотвратить перегрузки. В качестве критерия оптимальности используется сумма полезностей всех пользователей компьютерной сети.

Первоначально стандартные
задачи распределения ресурсов,
сводящиеся к максимизации
совокупной полезности производителей
при совместном использовании имеющихся
ресурсов, были рассмотрены в~\cite{kelly},
также задача распределения
ресурсов в компьютерных сетях 
исследовалась в недавней работе~\cite{rokhlin}.  Предложенные в монографии~\cite{arrow1958decentralization} механизмы децентрализованного распределения ресурсов с тех пор привлекают большое внимание в экономических исследованиях, см., например,~\cite{kakhbod2013resource, campbell1987resource, friedman1995complexity} и ссылки в них.  В данной работе, следуя~\cite{nesterov2018dual, ivanova2018composite}, мы рассматриваем различные мезанизмы корректировки цен. Практическую ценность предложенные подходы имеют за счёт своей децентрализованности, что означает,
что для установления и корректировки цены 
в отдельном соединении необходима только реакция пользователей, которые используют это соединение,
а не реакция всех пользователей сети. При
таком механизме корректировки все соединения действуют независимо. 

Кроме того, один из предложенных в статье подходов, основанный на использовании стохастического метода
проекции субградиента, обходит следующую проблему, возникающую в реальных сетях. Дело в том, что в реальных сетях пакеты с данными, которые поступают от пользователей на соединение, приходят не одновременно, поэтому на практике суммарный трафик на соединении неизвестен.  
Для решения этой проблемы предлагается использовать стохастические методы, для
работы которых требуется не точное значение суммарного трафика, а только его оценка,
которую можно получить на основе трафика одного
из пользователей. \evv{Идея
использовать для решения данной проблемы стохастический метод проекции субградиента предложена
в работе~\cite{rokhlin}.}

\subsection{Содержание}
Статья организована следующим образом.
В разделе \ref{problem_statement} описана постановка задачи и построение двойственной к ней. Также приводятся все необходимые предположения для прямой задачи. В разделе~\ref{fgm} рассматривается решение предложенной задачи быстрым градиентным методом Нестерова~\cite{Nesterov1983}, получена оценка сложности данного метода, которая имеет порядок  $O\left(\dfrac{1}{\sqrt{\varepsilon}}\right)$.  В разделе~\ref{stoch} описано решение данной задачи с использованием стохастического метода проекции субградиента и приведены оценки сложности, которые имеют порядок  $O\left(\dfrac{1}{\varepsilon^2}\right)$.  

В разделе~\ref{ellipsoids} описано решение задачи с использованием метода эллипсоидов, который хорошо подходит для задач небольшой размерности, также приведён алгоритм построения сертификата точности для данного метода. Приведены оценки сложности, которые имеют порядок  $O\left(m^2\ln\dfrac{1}{\varepsilon}\right)$,
где $m$~--- число соединений в сети. 
В разделе~\ref{reg} описана техника регуляризации, которая позволяет восстанавливать решение прямой задачи по решению двойственной для не прямо-двойственного метода. В разделе~\ref{RGEM} описано решение регуляризованной задачи с использованием метода экстраполяции случайного градиента.  Приведены оценки сложности, которые имеют порядок  $O\left(\dfrac{1}{\sqrt{\varepsilon}}\ln\dfrac{1}{\varepsilon}\right)$, где логарифмический множитель возникает за счёт регуляризации двойственной задачи.

В разделе~\ref{experim} приведено 
описание вычислительных экспериментов, подтверждающих на практике теоретические результаты, полученные в предыдущих разделах. 

 Также для каждого алгоритма описано его распределённое вычисление в контексте рассматриваемой задачи.

%\subsection{Обозначения}
%\ev{А куда пропало отсюда пояснение
%про скалярное произведение?}

%Кроме того, будет использоваться обозначение $\mu_+ = \max \{\mu, \, 0 \}$.









==> include/problem_statement.tex <==
\section{Постановка задачи}\label{problem_statement}
Рассмотрим компьютерную сеть с $m$ соединениями
и $n$ пользователями (или узлами),
см. рис.~\ref{fig:databaseUserTable}. 

\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-39pt}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{include/plots/gr3.png}
    \caption{Пример компьютерной сети с $m=6$  и $n=3$}
    \label{fig:databaseUserTable}
  \end{center}
\vspace{-25pt}
\end{wrapfigure}
Пользователи
обмениваются пакетами через фиксированный набор
соединений. 
Структура сети задана матрицей маршрутизации $C = (C_i^j) \, \in \, \RR^{m \times n}$.
Столбцы матрицы $\mathbf{C}_i \neq 0$, $i = 1, \, \ldots,
\, n$~--- булевы $m$-мерные векторы, такие, что
$C_i^j = 1$ в случае использования
узлом~$i$ соединения~$j$, в противном случае $C_i^j = 0$.
Ограничения на пропускную способность
соединений задаются вектором~$\mathbf{b} \, \in \, \RR^m$
со строго положительными компонентами.

Пользователи оценивают качество работы сети
с помощью функций полезности $u_k(x_k)$, $k = 1, \, \ldots, \, n$, где $x_k \, \in \, \RR_+$~-- скорость передачи данных $k$--го пользователя.
За критерий
оптимальности системы принята сумма функций полезностей для всех пользователей~\cite{kelly}.
%Управление ресурсами сети является децентрализованным: пользователи и соединения считаются узлами сети, 
%которые динамически обновляют
%(вычисляют) свои данные.

Задача максимизации суммарной полезности сети при заданных ограничениях на пропускную способность соединений формулируется следующим образом:
\begin{equation}
\label{eq_main_task}
    \max_{\left \{ C \mathbf{x} = \sum\limits_{k = 1}^n \mathbf{C}_k x_k \right \} \, \le \, \mathbf{b}} \left \{ U( \mathbf{x}) = \sum_{k = 1}^n u_k(x_k) \right \},
\end{equation}
где $\mathbf{x} = (x_1, \, \ldots, \, x_n) \, \in \, \mathbb{R}^n_+$.
Решением данной задачи будет оптимальное
распределение ресурсов~$\mathbf{x^*}$.



Рассмотрим стандартный переход к двойственной задаче
для~\eqref{eq_main_task}. Пусть задан вектор двойственных множителей $ \boldsymbol{\lambda} =
(\lambda_1, \, \ldots, \, \lambda_m) \, \in \, \mathbb{R}^m_+$, который можно интерпретировать как вектор цен соединений. Определим
двойственную целевую
функцию %\pd{Кажется, у $\sum_{k = 1}^n u_k(x_k)$ должен быть минус.}
\begin{equation}
\label{eq_phi_first}
\varphi(\boldsymbol{\lambda}) = \max_{\mathbf{x} \, \in \, \RR_+^n} 
\left \{
\sum_{k = 1}^n u_k(x_k) + \langle \boldsymbol{\lambda},
\mathbf{b} - \sum_{k = 1}^n \mathbf{C}_k x_k \rangle
\right \} =
\langle \boldsymbol{\lambda}, \mathbf{b} \rangle + \sum_{k = 1}^n (u_k(x_k(\boldsymbol{\lambda})) - \langle \boldsymbol{\lambda}, \, \mathbf{C}_k x_k(\boldsymbol{\lambda}) \rangle ),
\end{equation}
причём пользователи выбирают оптимальные скорости передачи
информации $x_k$, решая следующую задачу
оптимизации
\begin{equation}
\label{eq_xi_argmax}
x_k(\boldsymbol{\lambda})  =  \argmax_{x_k \, \in \, \RR_+} \left \{
u_k(x_k) - x_k \langle \boldsymbol{\lambda}, \, \mathbf{C}_k \rangle
\right \}.
\end{equation}
Обозначим также за $\pd{\mathbf{x}}(\boldsymbol{\lambda})$ вектор с компонентами $x_k(\boldsymbol{\lambda})$.
Тогда для нахождения оптимальных цен $\boldsymbol{\lambda^*}$
требуется решить задачу
\begin{equation}
\label{dual_problem}
\min_{\boldsymbol{\lambda} \, \in \, \RR_+^m} \varphi(\boldsymbol{\lambda}).
\end{equation}

Предположим, что для прямой задачи выполняется условие Слейтера, тогда в силу сильной двойственности и прямая, и двойственная задачи будут иметь решение. Используя условие Слейтера, можно компактифицировать решение двойственной задачи. Будем предполагать, что для решения двойственной задачи верна следующая оценка: 
$$
||\boldsymbol{\lambda}^*||_2 \leq R.
$$
При этом значение $R$ никак не влияет на работу рассматриваемых алгоритмов, а только присутствует в оценках скорости их сходимости. 

Основная идея данной работы заключается в применении различных оптимизационных методов для решения двойственной задачи~\eqref{dual_problem} с добавлением прямо-двойственного анализа этих методов, позволяющего также восстановить решение прямой задачи~\eqref{eq_main_task}. В этом смысле мы развиваем подход наших предыдущих работ \cite{gasnikov2016efficient,chernov2016fast,dvurechensky2016primal-dual,anikin2017dual,dvurechensky2018computational,nesterov2018primal-dual, guminov2019acceleratedAM,guminov2019accelerated,kroshnin2019complexity,uribe2018distributed,dvinskikh2019primal,dvurechensky2018decentralize}. Основное отличие состоит в рассмотрении ограничений-неравенств, а также в анализе стохастических алгоритмов в смысле оценок с большой вероятностью, а не в среднем. 

\subsection{Сильно вогнутые функции полезности}

В некоторых разделах мы будем предполагать, что
функции полезности $u_k(x_k)$, $k = 1, \, \ldots, \, n$, являются {\it сильно вогнутыми} с константой $\mu$. В данном подразделе опишем, какими свойствами будет обладать двойственная задача при таком предположении. 

\begin{Coro}~\textbf{(Теорема Демьянова--Данскина--Рубинова)}
\cite{Danskin, Dem_book_74}
\label{2_cor_dem}
Пусть для любого $\boldsymbol{\lambda} \, \in \, \mathbb{R}_+$ выполняется: $\varphi(\boldsymbol{\lambda})=\max \limits_{\mathbf{x} \in X} F(\mathbf{x}, \, \boldsymbol{\lambda})$, где $F(\mathbf{x}, \, \boldsymbol{\lambda})$~--- выпуклая и гладкая по $\boldsymbol{\lambda}$ функция и максимум достигается в единственной точке $x(\boldsymbol{\lambda})$. Тогда $\nabla \varphi(\boldsymbol{\lambda}) = 
\evv{\nabla_{\boldsymbol{\lambda}} F(x(\boldsymbol{\lambda}), \, \boldsymbol{\lambda})}
%\nabla F_{\boldsymbol{\lambda}}(x(\boldsymbol{\lambda}), \, \boldsymbol{\lambda})
$.
\end{Coro}

\begin{Coro} \cite{Nest}
\label{2_cor_sopr}
Пусть для любого $k = 1, \, \ldots, \, n$  функции $u_k(x_k)$ являются $\mu$-сильно вогнутыми.
Тогда функция (\ref{eq_phi_first}), где $x_k(\boldsymbol{\lambda}),\; k =1, \, \ldots, \, n$, являются решением задачи~\eqref{eq_xi_argmax}, будет $n m^2/\mu$-гладкой, т.е. градиент функции~$\varphi(\boldsymbol{\lambda})$
будет удовлетворять условию Липшица с константой $L= n m^2/\mu$: 
\begin{equation}
\label{2_smooth}
    \left|\left|\nabla \varphi(\boldsymbol{\lambda}^2)-\nabla\varphi(\boldsymbol{\lambda}^1)\right|\right|_2 \leqslant   L\left|\left|\boldsymbol{\lambda}^2 - \boldsymbol{\lambda}^1\right|\right|_2.
\end{equation}
\end{Coro}
Доказательство утверждения можно найти в Приложении. 


\subsection{Вогнутые функции полезности}
Теперь предположим, что функции полезности $u_k(x_k)$, $k = 1, \, \ldots, \, n$, являются {\it вогнутыми, но не сильно вогнутыми}. Тогда двойственная задача не является гладкой. В данном подразделе описаны некоторые свойства субградиентов двойственной задачи при таких предположениях.

Субградиент двойственной задачи~\eqref{dual_problem} определяется следующим образом: 
\begin{equation*}
\ev{\nabla} \varphi(\boldsymbol{\lambda} )=
\mathbf{b} - C\mathbf{x}.
\end{equation*}
Учитывая, что $\mathbf{x}$~--- ограниченная скорость передачи информации и вектор~$\mathbf{b}$ также ограничен, получаем, что субградиенты двойственной задачи в данном случае ограничены. Таким образом, существует такая положительная константа~$M$, что верна следующая оценка
\begin{equation}
\label{eq_gradM}
 \| \ev{\nabla}%\partial 
 \varphi(\boldsymbol{\lambda} ) \|_2
\, \le \, M.
\end{equation}
\evv{В качестве грубой оценки сверху для константы~$M$ из~\eqref{eq_gradM}  можно использовать $O(n\sqrt{m})$. Множитель~$n$ возникает из-за того, что есть $n$~слагаемых, а $\sqrt{m}$ 
используется как оценка зависимости
$2$-нормы от размерности вектора~$m$. }


==> include/reg.tex <==
\section{Регуляризация двойственной задачи}
\label{reg}
В предыдущих параграфах мы рассматривали прямо-двойственные методы для решения двойственной задачи. Однако существует стандартный подход, который позволяет по решению двойственной задачи не прямо-двойственным методом воостанавливать решение прямой задачи. Ключевой идеей данного подхода является регуляризация двойственной задачи, которая гарантирует сильную выпуклос\ev{т}ь регуляризованной задачи. Далее опишем подробно предлагае\ev{м}ый подход и сформулируем леммы, связывающие решения прямой  и двойственной задачи. 

Регуляризуем функционал \eqref{eq_phi_first} по А.Н. Тихонову:
$$
    \varphi_\delta(\boldsymbol{\lambda}) = \varphi(\boldsymbol{\lambda}) + \frac{\delta}{2}\|\boldsymbol{\lambda}\|^2_2
$$
и вместо задачи \eqref{dual_problem} будем решать регуляризованную задачу
\begin{equation} \label{regularized}
    \min_{\boldsymbol{\lambda} \, \in \, \RR_+^m} \varphi_{\delta}(\boldsymbol{\lambda}).
\end{equation}
Параметр $\delta$ будет оптимально подобран позже. Как и в предыдущем параграфе, предполагается, что задача решается на множестве
$$
\Lambda_{2R} = \{\boldsymbol{\lambda} \in \mathbb{R}_{+}^m: \|\boldsymbol{\lambda}\|_2 \leq 2 R\}.
$$
Для полученной регуляризованной функции сформулируем следующу\ev{ю} лемму о гладкости регуляризованной задачи. 
\begin{Lem}\label{lem_reg_continuity}
% \ai{Эту лемму лучше сформулировать "Пусть функция $\varphi$ $L$-гладкая, тогда регуляризованная является $L+\delta$ гладкой и доказательство привести..доказательство начинается аналогично тому, что ты в примечании написал. И далее составшись на утверждение 1 сказать что будет в нашей задаче.} 
Пусть функция $\varphi(\boldsymbol{\lambda})$~--- $L$-гладкая, тогда регуляризованная функция $\varphi_\delta(\boldsymbol{\lambda})$ является $(L+\delta)$-гладкой, т.е. \ev{для любых $\boldsymbol{\lambda}^1$, $\boldsymbol{\lambda}^2 \, \in \, \RR_+^m$}
\begin{equation} \label{regularized_continuity}
\left \|\nabla \varphi_\delta(\boldsymbol{\lambda}^1) - \nabla \varphi_\delta(\boldsymbol{\lambda}^2) \right \|_2 \leq (L + \delta) \left \|\boldsymbol{\lambda}^1 - \boldsymbol{\lambda}^2 \right \|_2.
\end{equation}
% Из сильной выпуклости функций полезности $u_i(x^i), i=1, ..., N$ следует, что функционал $\varphi(\lambda)$ является гладким:
% $$
% \|\nabla \varphi(\lambda_1) - \nabla \varphi(\lambda_2)\|_2 \leq L \|\lambda_1 - \lambda_2\|_2, 
% $$
% и регуляризованный функционал $\varphi_\delta(\lambda)$ является гладким с константой Липшица градиента равной $L + \delta$:
% $$
% \|\nabla \varphi_\delta(\lambda_1) - \nabla \varphi_\delta(\lambda_2)\|_2 \leq (L + \delta) \|\lambda_1 - \lambda_2\|_2.
% $$
\end{Lem}
\textbf{Доказательство.} Градиент регуляризованной функции $\nabla \varphi_\delta(\boldsymbol{\lambda}) = \nabla \varphi(\boldsymbol{\lambda}) + \delta \boldsymbol{\lambda}$. Следовательно, имеем следующую оценку
$$
\left \|\nabla \varphi_\delta(\boldsymbol{\lambda}^1) - \nabla \varphi_\delta(\boldsymbol{\lambda}^2) \right \|_2
= \left \|\nabla \varphi(\boldsymbol{\lambda}^1) - \nabla \varphi(\boldsymbol{\lambda}^2) + \delta (\boldsymbol{\lambda}^1 - \boldsymbol{\lambda}^2) \right \|_2 \leq \left \|\nabla \varphi(\boldsymbol{\lambda}^1) - \nabla \varphi(\boldsymbol{\lambda}^2) \right \|_2 +
$$
$$
+ \delta \left \|\boldsymbol{\lambda}^1 - \boldsymbol{\lambda}^2 \right \|_2.
$$
Откуда \ev{в силу У}тверждения~\ref{2_cor_sopr} следует \eqref{regularized_continuity}. $\quad \blacksquare$

Также для оценки сходимости \ev{алгоритма для } прямой задачи нам понадобится следующая вспомогательная лемма
%, которая помогает установить
\ev{o связи} между оценкой на градиент для двойственной задачи и оценками на сходимость по функции и невязку в ограничении для прямой задачи. 
% \ai{пусть лучше * всегда будут как верхний индекс, чтобы везде одинаково было}
\begin{Lem}{\cite{Gasnikov2016ELP}} \label{lem_regularized_dual}
Пусть $\mathbf{x}^{*}$~--- решение прямой задачи \eqref{eq_main_task}. Тогда
\ev{выполняются следующие неравенства:}
\begin{equation} \label{eq_limits_reg1}
    \|C \mathbf{x}(\boldsymbol{\lambda}) - \mathbf{b}\|_2 \leq \|\nabla \varphi_\delta (\boldsymbol{\lambda})\|_2 + \delta \|\boldsymbol{\lambda}\|_2,
\end{equation}
\begin{equation} \label{eq_err_reg1}
     U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda})) \leq \|\nabla \varphi_\delta(\boldsymbol{\lambda})\|_2 \cdot \|\boldsymbol{\lambda}\|_2 + \delta \|\boldsymbol{\lambda}\|_2^2,
\end{equation}
где $\mathbf{x}(\boldsymbol{\lambda})$ определяется \ev{в} \eqref{eq_xi_argmax}. 
\end{Lem}
\textbf{Доказательство.}
%По определению $\mathbf{x}(\boldsymbol{\lambda})$, имеем
\ev{В силу \eqref{eq_xi_argmax}}
$$
U(\mathbf{x}(\boldsymbol{\lambda})) + \langle \boldsymbol{\lambda}, \, \mathbf{b} - C \mathbf{x}(\boldsymbol{\lambda}) \rangle \geq U(\mathbf{x}^{*}) + \langle \boldsymbol{\lambda}, \, \mathbf{b} - C \mathbf{x}^{*} \rangle \geq U(\mathbf{x}^{*}).
$$
Откуда
$$
U(\mathbf{x}(\boldsymbol{\lambda})) \geq U(\mathbf{x}^{*}) - \langle \boldsymbol{\lambda}, \, \mathbf{b} - C \mathbf{x}(\boldsymbol{\lambda}) \rangle = U(\mathbf{x}^{*}) - \langle \boldsymbol{\lambda}, \, \nabla \varphi(\boldsymbol{\lambda}) \rangle.
$$
% \ai{лучше просто вынести выкладки из примечания без ссылки на лемму из статья Гасников и др.}
Так как $\varphi(\boldsymbol{\lambda}) = \varphi_\delta(\boldsymbol{\lambda}) - \frac{\delta}{2} \|\boldsymbol{\lambda}\|_2^2$, имеем
$$
\|\nabla \varphi(\boldsymbol{\lambda}) \|_2 = \|\nabla \varphi_\delta(\boldsymbol{\lambda}) - \delta \boldsymbol{\lambda}\|_2 \leq \|\nabla \varphi_\delta(\boldsymbol{\lambda})\| + \delta \|\boldsymbol{\lambda}\|_2.
$$
% \textcolor{brown}{Примечание: как я понял, это неравенство остаётся неизменным, несмотря на то, что в статье Гасников и др. там $-\frac{\delta}{2} \|\lambda\|^2$, а у нас $+\frac{\delta}{2} \|\lambda\|^2$. В этом я руководствовался следующими выкладками:
% $$
% \varphi = \varphi_\delta - \frac{\delta}{2} \|\lambda\|^2 \Rightarrow \|\nabla \varphi\| = \|\nabla \varphi_\delta - \delta \lambda\| \leq \|\nabla \varphi_\delta\| + \delta \|\lambda\|
% $$}
\ev{Из последнего неравенства}, учитывая соотношение $\nabla \varphi(\boldsymbol{\lambda}) = \mathbf{b} - C \mathbf{x}(\boldsymbol{\lambda})$, получаем \eqref{eq_limits_reg1}. 

Далее, оценка \eqref{eq_err_reg1} следует из 
%следующей выкладки
$$
U(\mathbf{x}^{*}) - U(\mathbf{x}(\boldsymbol{\lambda})) \leq \langle \boldsymbol{\lambda}, \, \nabla \varphi(\boldsymbol{\lambda}) \rangle \leq \|\nabla \varphi(\boldsymbol{\lambda})\|_2 \cdot \|\boldsymbol{\lambda}\|_2 \leq 
$$
$$
\qquad \leq \|\boldsymbol{\lambda}\|_2 \cdot \left ( \left \|\nabla \varphi_\delta(\boldsymbol{\lambda}) \right \|_2 + \delta \left \|\boldsymbol{\lambda} \right \|_2 \right ) \leq \|\nabla \varphi_\delta(\boldsymbol{\lambda})\|_2 \cdot \|\boldsymbol{\lambda}\|_2 + \delta \|\boldsymbol{\lambda}\|_2^2. \quad \blacksquare
$$
Кроме этого, понадобится лемма о сходимости по градиенту для регуляризованной функции.
\begin{Lem} \label{lem_reqularized_ineqs}
\ev{Пусть $\boldsymbol{\lambda}_\delta^{*}$~--- решение регуляризованной двойственной задачи.}
Име\ev{e}т место следующее неравенство
$$
   \left \|\nabla \varphi_\delta(\boldsymbol{\lambda}^{N}) \right \|_2 \leq (L + \delta) \left \|\boldsymbol{\lambda}^{N} - \boldsymbol{\lambda}_\delta^{*} \right \|_2.
$$
%$$
    %\varphi_\delta(\boldsymbol{\lambda}_1) - \varphi_\delta(\boldsymbol{\lambda}_\delta^{*}) \leq (L + \delta) \left(\|\boldsymbol{\lambda}_1\|_2^2 + \|\boldsymbol{\lambda}_\delta^{*}\|_2^2\right)
%$$
\end{Lem}
\textbf{Доказательство}
% \ai{сослаться на Лемму 2 (она как раз про гладкость) и просто написать, что учитывая что $\nabla \varphi_{delta}(\lambda^*_{delta}) = 0$, получаем....}
% Первое неравенство следует из гладкости фукнционала $\varphi_\delta(\boldsymbol{\lambda})$
\ev{ немедленно следует из Леммы \ref{lem_reg_continuity} и 
%Из Леммы \ref{lem_reg_continuity} имеем %\eqref{regularized_continuity}, откуда, учитывая 
равенства~$\nabla \varphi_\delta(\boldsymbol{\lambda}^{*}_\delta) = 0$.}
$\blacksquare$
%, получаем

% $$
% \|\nabla \varphi_\delta(\boldsymbol{\lambda}_{T+1})\| = \|\nabla \varphi_\delta(\boldsymbol{\lambda}_{T+1}) - \nabla \varphi_\delta(\boldsymbol{\lambda}_\delta^{*})\| \leq (L + \delta) \|\boldsymbol{\lambda}_{T+1} - \boldsymbol{\lambda}_\delta^{*}\|
% $$
%$$
%\|\nabla \varphi_\delta(\boldsymbol{\lambda}^{N})\|_2 \leq (L + \delta) \|\boldsymbol{\lambda}^{N} - \boldsymbol{\lambda}_\delta^{*}\|_2. \quad \blacksquare
%$$

Мы сформулировали необходимые леммы для регуляризованной задачи и в следующем параг\ev{р}афе рассмотрим на примере применение этого подхода. 

==> include/stoch.tex <==
\section{Стохастический метод проекции субградиента}
\label{stoch}
Рассмотрим исходную задачу~\eqref{eq_main_task},
но теперь предположим, что
функции полезности $u_k(x_k)$, $k = 1, \, \ldots, \, n$,
{\it вогнуты, но не сильно вогнуты}.
В этом случае двойственная
задача~\eqref{dual_problem}
становится негладкой.
Поэтому для её решения предлагается
применить стохастический метод проекции субградиента.
\evv{Впервые идея
использовать для решения данной проблемы стохастический метод проекции субградиента предложена
в работе~\cite{rokhlin}.}

Рассмотрим вероятностное пространство $\left(\Omega, \, \mathcal F, \, \PP \right)$. Пусть на нём определена последовательность независимых случайных величин $\{\xi^t \}_{t=0}^{\infty}$, равномерно распределённых на $\{1, \,
\ldots, \, n\}$, т.е.
$$
\PP(\xi^{t}=i) = \dfrac{1}{n}, \, \, \, i \, \in \, \{1, \, \ldots, \, n\}.
$$

Если доступен оракул, выдающий
стохастический субградиент двойственной функ\-ции~$\nabla \varphi(\boldsymbol{\lambda}, \, \xi)$:
$$
\nabla \varphi(\boldsymbol{\lambda}, \, \xi) =\mathbf{b}- \pd{n}C_{\xi}x_{\xi}(\boldsymbol{\lambda}), %\pd{\text{Тут наверное у $x$ должен индекс быть внизу.}}
$$
то
$$
\EE \left [\mathbf{b}- nC_{\xi_{t}}x_{\xi_{t}}(\boldsymbol{\lambda}^t) \, | \, \xi^{t} \right ] =
\mathbf{b}- \sum\limits_{k=1}^{n} \mathbf{C}_{k}x_{k}(\boldsymbol{\lambda}^t) = \nabla \varphi(\boldsymbol{\lambda}^t)
$$
Следовательно, стохастический субградиент является несмещённой оценкой субградиента. 

 %Определим вектор $\mathbf{x}(\boldsymbol{\lambda}^t, \xi^{t}) = [0,
%\, \ldots, \, \underbrace{n %x_{\xi^{t}}(\boldsymbol{\lambda}^t)}_{\xi^{t}}, \, \ldots, \, 0 ]^{T}$. 

%\floatname{algorithm}{Алгоритм}
	\begin{algorithm}
		\caption{Прямо-двойственный стохастический метод проекции субградиента~(PDSSGM), версия~1}\label{alg_stoch} 
		\begin{algorithmic}[1]
			
			\Require $u_k(\mathbf{x}), \; \; k=1, \, \ldots, \, n$~--- вогнутые функции полезности для каждого пользователя;
			$\beta$~--- шаг метода.
			%\Ensure цена $p^N$, для которой выполняется $\left|C-\sum \limits_{k=1}^n x_k(p^N)\right|\leqslant   \varepsilon$.
			\State $\boldsymbol{\lambda}^0 := \mathbf{0}$
			\For{$t= 1, \, \ldots, \, N-1$}
			\State Вычислить $\nabla \varphi(\boldsymbol{\lambda}^{t-1}, \, \xi)$
			\State $\boldsymbol{\lambda}^{t} := [\boldsymbol{\lambda}^{t-1} - \beta \left(\mathbf{b}- nC_{\xi^{t-1}}x_{\xi^{t-1}}(\boldsymbol{\lambda}^{t-1}) \right)]_+$
			\State $\hat{ \mathbf{x}}^{t+1} := \dfrac{1}{t+1}
			\sum\limits_{j=0}^{t}\mathbf{x}(\boldsymbol{\lambda}^j) $ 
			\State $\hat{\boldsymbol{\lambda}}^{t+1} := \dfrac{1}{t+1}\sum\limits_{j=0}^{t}\boldsymbol{\lambda}^j $
             \EndFor
			\State\Return $\hat{\boldsymbol{\lambda}}^{N}, \hat{ \mathbf{x}}^{N}$
		\end{algorithmic}
	\end{algorithm}


Оптимальное решение задачи~\eqref{eq_phi_first} будем
искать с помощью 
прямо-двойственного стохастического метода
проекции субградиента~PDSSGM. 
Приведём описание двух версий данного метода,
см. Алгоритм~\ref{alg_stoch} и Алгоритм~\ref{alg_stoch_1}. 
В Алгоритме~\ref{alg_stoch} используется полная модель восстановления вектора~$\mathbf{x}(\boldsymbol{\lambda})$ на каждой итерации. \pd{Однако, вычисление вектора $\mathbf{x}(\boldsymbol{\lambda})$ по сложности практически эквивалентно вычислению полного субградиента $\varphi(\boldsymbol{\lambda} )$. Поэтому основным алгоритмом является  Алгоритм~\ref{alg_stoch_1}, в котором} для восстановления вектора~$\mathbf{x}(\boldsymbol{\lambda})$ используется неполная, стохастическая модель, 
что означает, что на каждой итерации пересчитывается только одна компонента вектора~$\mathbf{x}(\boldsymbol{\lambda})$, остальные остаются без изменений. \pd{При доказательстве теоремы сходимости мы сначала показываем оценку скорости сходимости для Алгоритма~\ref{alg_stoch}, а затем показываем, что приближённое решение прямой задачи, полученное в Алгоритме~\ref{alg_stoch_1}, близко по точности к решению, полученному в Алгоритме~\ref{alg_stoch}.}



\begin{algorithm}
		\caption{Прямо-двойственный стохастический метод проекции субградиента~(PDSSGM), версия~2}\label{alg_stoch_1}
		\begin{algorithmic}[1]
			
			\Require $u_k(\mathbf{x}), \; \; k=1, \, \ldots, \, n$~--- вогнутые функции полезности для каждого пользователя;
			$\beta$~--- шаг метода.
			%\Ensure цена $p^N$, для которой выполняется $\left|C-\sum \limits_{k=1}^n x_k(p^N)\right|\leqslant   \varepsilon$.
			\State $\boldsymbol{\lambda}^0 := \mathbf{0}$
			\For{$t= 1, \, \ldots, \, N-1$}
			\State Вычислить $\nabla \varphi(\boldsymbol{\lambda}^{t-1}, \, \xi)$
			\State $\boldsymbol{\lambda}^{t} := [\boldsymbol{\lambda}^{t-1} - \beta \left(\mathbf{b}- nC_{\xi^{t-1}}x_{\xi^{t-1}}(\boldsymbol{\lambda}^{t-1}) \right)]_+$
			\State $\Tilde{\mathbf{x}}^{t+1}_{\xi^t} := \frac{t}{t+1}\Tilde{\mathbf{x}}^{t}_{\xi^t} + \frac{1}{t+1}n x_{\xi^{t}}(\boldsymbol{\lambda}^{t})$, 
			\quad
			$\Tilde{\mathbf{x}}^{t+1}_{j} := \Tilde{\mathbf{x}}^{t}_j$ \mbox{ при } $j\neq \xi^t$ 
			\State $\hat{\boldsymbol{\lambda}}^{t+1} := \dfrac{1}{t+1}\sum\limits_{j=0}^{t}\boldsymbol{\lambda}^j $
             \EndFor
			\State\Return $\hat{\boldsymbol{\lambda}}^{N}, \Tilde{\mathbf{x}}^{N}$
		\end{algorithmic}
	\end{algorithm}
	
	

% \pd{Что такое $\mathbf{x}(\boldsymbol{\lambda})$?}
	
\subsection{Распределённый метод}
Рассмотрим, как
можно применить для решения рассматриваемой задачи
стохастический 
метод проекции субградиента в распределённом варианте. 

Опишем процесс, происходящий на $t$-ой итерации для соединения~$j$:

1. На основе информации, полученной 
от соединений после предыдущей итерации с номером~$t-1$, случайный пользователь $\xi^t$ передает данные с оптимальной скоростью 
$$
x_{\xi^t}(\boldsymbol{\lambda}^{t+1}) = \argmax_{x_{\xi^t} \, \in \, \RR_+} \left (
u_{\xi^t}(x_{\xi^t}) - x_{\xi^t} \sum_{j = 1}^m \lambda^{t+1}_j C_{\xi^t}^j
\right ),
$$
где в силу определения матрицы $C$ пользователю необходима информация только от соединений, которые он использует.

2. Далее соединение $j$ вычисляет цену на следующую итерацию на основе реакции этого пользователя
$$\lambda^{t + 1}_j = \left[\lambda_{j}^t -
			\beta
			\left ( b_j - n C_{\xi^t}^j x_{\xi^t}^t \right )\right]_{+}.$$
При этом $C_{\xi^t}^j \neq 0$ только для тех пользователей, которые используют соединение $j$. Поэтому цена поменяется только для 
актуальных \evv{соединений} пользователя, который передал данные.


Замечание. {\it Главное преимущество данного метода заключается в том, что соединение меняет цену только на основе реакции одного пользователя, что гораздо
больше приближает
постановку задачи к ситуации
в реальных сетях, в которых пользователи отправляют данные не одновременно.}

\subsection{Оценка скорости сходимости для стохастического метода проекции субградиента}

\ai{Прежде чем перейти к доказательству основной теоремы об оценках скорости сходимости предложенных методов\ev{,} приведём необходимые предположения \ev{для решаемой задачи}.
Предположим, что существует положительная константа~$M  = O( n \sqrt{m})$, такая, что верна следующая оценка:
\begin{equation}
\label{eq_stoch_gradM}
 \| \nabla \varphi(\boldsymbol{\lambda}, \, \xi) \|_2 
\, \le \, M.
\end{equation}
Данное предположение корректно в силу того, что скорость передачи информации~$\mathbf{x}$ ограничена и вектор пропускных способностей~$\mathbf{b}$ также ограничен в силу физических соображений. Поэтому, исходя из определения стохастического субградиента, %получаем, что
он ограничен. 
}
%\pd{Из абзаца ниже не очень понятно, какое все-таки предположение про $M$ мы делаем. По идее в нашем случае можно $M$ оценить. Предположения про $M$, $\sigma$ лучше перенести поближе к теоремам.}
%В силу того, что скорость передачи информации~$\mathbf{x}$ ограничена  и вектор~$\mathbf{b}$ также ограничен,  стохастический субградиент двойственной задачи ограничен. Предположим, что существует положительная константа~$M  = O( n)$, такая, что верна следующая оценка:
%\begin{equation*}
%\EE \left [ \| \nabla \varphi(\boldsymbol{\lambda}, \, \xi) \|_2^2 %\right ]
%\, \le \, M^2.
%\end{equation*}
%При выполнении более сильного неравенства
%$$
%\EE\left[\exp\left(\frac{\| \nabla \varphi(\boldsymbol{\lambda}, \, \xi)\|_2^2}{M^2}\right)\right] \le \exp(1)
%$$
%будет верным 
%\begin{equation}
%\label{eq_stoch_gradM}
% \| \nabla \varphi(\boldsymbol{\lambda}, \, \xi) \|_2 
%\, \le \, M.
%\end{equation}
%\pd{Вроде же наборот, из ограниченности следуют экспоненциальные моменты.} \ai{вроде того, что наверху достаточно и про ограниченность моментов можно не писать}

Также предположим, что
$$
\pd{\mathbb{E}}
\left [ 
\exp
\left (
\frac{\left \| \nabla \varphi(\boldsymbol{\lambda}, \, \xi) -
\nabla \varphi(\boldsymbol{\lambda})
\right \|^2_2 }{\sigma^2}
\right )
\right ]\, \le \, \exp(1),
%\left \| \mathbb{E} [\nabla \varphi(\boldsymbol{\lambda}, \, \xi)] -
%\nabla \varphi(\boldsymbol{\lambda}, \, \xi)
%\right \|^2_2 
%\right ]\, \le \, \sigma^2,
$$
где $\sigma$~--- положительная числовая константа, \evv{порядок зависимости от $n$ и $m$ такой же, как у $M$}.


Для получения оценки скорости сходимости Алгоритма~\ref{alg_stoch_1} необходимо предположение о том, что {\it функции $u_k(x_k), \, k = 1, \, \ldots, \, n$ являются липшицевыми с константой~$M_{u_k}$}, тогда функция~$U(\mathbf{x})$ будет липшицевой
с некоторой константой~$M_{U}$:
$$
\forall \, \mathbf{x}, \, \mathbf{y} \quad
   |U(\mathbf{x}) - U(\mathbf{y})| \leq M_{U}\|\mathbf{x} - \mathbf{y} \|_2,
$$
при этом $M_{U} = O(\sqrt{n})$.
Может оказаться, что функция $u_k(x_k)$ липшицева везде, кроме, например, точки~$0$. Примером такой функции является
одна из наиболее распространённых функций полезности пользователей~$u_k(x_k) = \ln x_k$. 
%Соответственно в $0$ логарифм имеет неошграниченную производную. 
Но в силу специфики рассматриваемой задачи 
%можно считать, что 
всегда существуют $\bar{\varepsilon} > 0$,  $\underline{\varepsilon} >0$, такие, что $x^*_k \, \geq \, \underline{\varepsilon}$, $x^*_k \, \leq \, \bar{\varepsilon}$. Тогда 
задачу можно решать на компакте~$Q = \left \{ \mathbf{x} \, : \, \underline{\varepsilon} \leq x_k \leq \bar \varepsilon, \, k = 1, \, \ldots, \, n \right \}$,
и рассматриваемая функция~$u_k(x_k) = \ln x_k$ становится липшицевой на~$Q$. В общем случае 
вогнутая функция полезности~$u(x)$ будет липшицевой
на компакте, лежащем в относительной внутренности
области определения~$u(x)$.
% EV: мне кажется, для липшицевости выпуклой
% функции нужна ограниченность и сверху,
% поэтому я добавила её

\ev{Пусть}%Обозначим
$$
\mathbb{E}
\left [ 
\exp
\left (
\frac{\left \|\mathbf{x}(\boldsymbol{\lambda}, \, \xi) -
\mathbf{x}(\boldsymbol{\lambda})
\right \|^2_2 }{\sigma_x^2}
\right )
\right ]\, \le \, \exp(1),
%\left \| \mathbb{E} [\nabla \varphi(\boldsymbol{\lambda}, \, \xi)] -
%\nabla \varphi(\boldsymbol{\lambda}, \, \xi)
%\right \|^2_2 
%\right ]\, \le \, \sigma^2,
$$
где $\sigma_x = O(\sqrt{n})$~--- положительная числовая константа и $\mathbf{x}(\boldsymbol{\lambda}, \, \xi) = (0, \, \ldots, \, n x_{\xi}(\boldsymbol{\lambda}), \, \ldots, \, 0)^{T}$.

Сформулируем ключевую лемму, необходимую для получения оценок скорости сходимости невязки в ограничениях и зазора двойственности 
после работы прямо-двойст\-вен\-ного метода~PDSSGM.

\begin{Lem}
\label{lem_stoch_main}
Пусть Алгоритм~\ref{alg_stoch_1} начинает свою работу с начальной точки $\boldsymbol{\lambda}^0=\mathbf{0}$
и с шагом~$\beta$.
Тогда после $N$ итераций Алгоритма~\ref{alg_stoch_1}
с вероятностью $1 - 4\delta$ 
выполняется неравенство:
 \begin{eqnarray*}
 \varphi(\boldsymbol{\hat{\lambda}}^N) 
&  - &  U(\Tilde{\mathbf{x}}^N)  + 
2 R
\left \|
\left [C \Tilde{\mathbf{x}}^N - \mathbf{b}
\right ]_+ 
\right \|_2   \le    C_1\dfrac{R^2 \sigma\sqrt{ g(N)J} }{\sqrt{N}} 
+ \frac{2 R^2}{\beta N} +
\frac{\beta M^2}{2}  \notag \\ & + &    \frac{ \sqrt{2} \left (1 + \sqrt{3 \ln \frac{1}{\delta}} \right )}{\sqrt{N}}  \left( M_{U} \sigma_x + 2R\left(\sigma + \sigma_x \sqrt{\lambda_{max}\left( C^{T}C \right)} \right) \right)\ev{,}
 \end{eqnarray*}
где $\hat{\boldsymbol{\lambda}}^N = \dfrac{1}{N} \sum\limits_{t=0}^{N-1}\boldsymbol{\lambda}^t$ и $\Tilde{\mathbf{x}}^N = \dfrac{1}{N} \sum\limits_{t=0}^{N-1}\mathbf{x}(\boldsymbol{\lambda}^t, \xi^{t}) $, $C_1$-- положительная числовая константа, %\pd{Думаю, стоит пояснить, что за природа константы $D$.}
$g(N) = \ln\left(\frac{N}{\delta}\right) + \ln\ln\left(\frac{F}{f}\right)$,
$$
F  = 2\sigma^2 N (2 \beta)^{N}\left(2R^2 + 2\beta^2 M^2 +  \beta R^2 + 24 \ln\frac{N}{\delta} \beta \sigma^2 N \right),
$$
$f = \sigma^2 R^2$  и 
$$
J = \max\left\{1, \quad \frac{1}{R} \beta C_1\sqrt{\sigma^2 g(N)} + \sqrt{\frac{1}{R^2} \beta^2 C_1^2\sigma^2g(N) + \frac{2R^2 + 2\beta^2 M^2}{R^2} }\right\},
$$
\ev{а} $R$ определяется \ev{условием } $||\boldsymbol{\lambda}^*||_2 \leq R$.
%\pd{Что такое $\sigma_x$, $R$?} \ai{Ввела наверху обозначение $\sigma_x$, а $R$ вводилось в постановке задачи тлт лучше еще раз ввести? } \pd{Лучше еще раз напомнить.}
\end{Lem}
Доказательство леммы приведено в Приложении.

Теперь сформулируем теорему об оценке скорости сходимости Алгоритма~\ref{alg_stoch_1}.
\begin{theorem}
Пусть Алгоритм~\ref{alg_stoch_1} начинает свою работу
с начальной точки $\boldsymbol{\lambda}^0=\mathbf{0}$
и с шагом~$\beta =\frac{R}{M\sqrt{N}}$. Обозначим $A=  \sqrt{2} \left (1 + \sqrt{3 \ln \frac{1}{\delta}} \right )  \left( M_{U} \sigma_x + 2R\left(\sigma + \sigma_x \sqrt{\lambda_{max}\left( C^{T}C \right)} \right) \right) + 2.5 RM$.
Тогда после %\pd{Не очень понятно. $N$ присутствует и слева и справа а равенстве.}
\begin{equation*}
N = O\left( \left \lceil \dfrac{A^2}{\varepsilon^2} \ln\left(\dfrac{MR}{\varepsilon\delta} \right) \right \rceil\right)
\end{equation*}
%\pd{не очень понятно, почему в оценку не входят $\sigma$, $\sigma_x$, $M_U$.}
итераций Алгоритма~\ref{alg_stoch_1} с вероятностью $1-4\delta$ будут
выполняться следующие неравенства: 
\begin{equation*}
U(\mathbf{x^*}) - U(\Tilde{\mathbf{x}}^{N}) \,  \le \, \varepsilon, \, \, \, \, 
  \left \| \left (C \Tilde{\mathbf{x}}^N - \mathbf{b} \right)_{+}\right \|_2 \, \le \, \frac{\varepsilon}{ R},
\end{equation*}
где $\Tilde{\mathbf{x}}^N = \frac{1}{N}
\sum\limits_{t = 0}^{N-1} \mathbf{x}(\boldsymbol{\lambda}^t, \xi^{t}) $,
$\mathbf{x^*}$ ~--- оптимальное решение задачи~\eqref{eq_main_task}.
%$A_1, \,  A_2, \, $ -- положительные константы, которые зависят от $R$  и $\delta$.
\end{theorem}
\textbf{Доказательство.}
Начало доказательства  
такое же, как в теореме~\ref{main_th_fgm}, но с использованием оценки из леммы~\ref{lem_stoch_main}. В результате, для шага~$\beta=\dfrac{R}{M\sqrt{N}}$ получим, что 
\begin{eqnarray*}
 \frac{ \sqrt{2} \left (1 + \sqrt{3 \ln \frac{1}{\delta}} \right )}{\sqrt{N}}  \left( M_{U} \sigma_x + 2R\left(\sigma + \sigma_x \sqrt{\lambda_{max}\left( C^{T}C \right)} \right) \right)
+ 
\frac{5R M}{2\sqrt{N}}  +    C_1\dfrac{
R ^ 2 \sigma\sqrt{ g(N)J} }{\sqrt{N}},
 \end{eqnarray*}
при этом с точностью до констант $g(N) \approx \ln\left(\frac{N}{\delta}\right)$, $J \approx \max
\left \{1, \, \beta\sqrt{g(N)} \right \}$. \pd{Далее найдем $N$, при котором оценка становится меньше $\varepsilon$.}

Введём следующие обозначения\ev{:}
$$
A=  \sqrt{2} \left (1 + \sqrt{3 \ln \frac{1}{\delta}} \right )  \left( M_{U} \sigma_x + 2R\left(\sigma + \sigma_x \sqrt{\lambda_{max}\left( C^{T}C \right)} \right) \right) + 2.5 RM, \quad B= C_1 R^2 \sigma.
$$
Необходимо получить минимальную оценку
\ev{на} число итераций~$N$ \pd{для} достижения
заданной точности~$\varepsilon$. Для $J=1$ получаем, что 
\begin{equation}
\label{eq_stoch_teor_estN}
\sqrt{N} =\left \lceil \dfrac{A+B\sqrt{\ln\left(\frac{N}{\delta}\right)}}{\varepsilon} \right \rceil.
\end{equation}
Подставляя рекурсивно значение $N$, из
\eqref{eq_stoch_teor_estN} получим следующую оценку сложности: 
$$
N = O \left(\left \lceil \dfrac{A^2}{\varepsilon^2} \ln\left(\dfrac{MR}{\varepsilon\delta} \right) \right \rceil \right).
$$

Для $J=\beta \sqrt{g(N)}=\dfrac{R\sqrt{g(N)}}{M\sqrt{N}}$
%и учитывая, что $J \leq J^2$ 
потребуем, чтобы
$$
\dfrac{A}{\sqrt{N}} + \dfrac{B g(N) R}{M N} = \dfrac{A}{\sqrt{N}} + \dfrac{\bar B g(N) }{N} \leq \varepsilon.
$$
Так как нам нужно найти минимальное $N$, то, заменив последнее неравенство на равенство и решая полученное уравнение, получаем, что 
$$
\sqrt{N} =\left \lceil \frac{A + \sqrt{A^2 + 4\varepsilon\bar B \ln\left(\frac{N}{\delta}\right) }}{2\varepsilon} \right \rceil.
$$
Аналогично случаю $J = 1$, из последнего
равенства получается следующая оценка: 
$$
N = O \left(\left \lceil \dfrac{A^2}{\varepsilon} \ln\left(\dfrac{MR}{\varepsilon\delta} \right) \right \rceil \right).
$$
Худшая из оценок сложности для $J = 1$ и для $J=\beta \sqrt{g(N)}$ и будет оценкой из условия теоремы.  $\blacksquare$




